Boda-RTC: Productive Generation of Portable, Efficient Code for Convolutional Neural Networks on Mobile Computing Platforms

The popularity of neural networks (NNs) spans academia, industry, and popular culture. In particular, convolutional neural networks (CNNs) have been applied to many image based machine learning tasks and have yielded strong results. The availability of hardware/software systems for efficient training and deployment of large and/or deep CNN models has been, and continues to be, an important consideration for the field. Early systems for NN computation focused on leveraging existing dense linear algebra techniques and libraries. Current approaches use low-level machine specific programming and/or closed-source, purpose-built vendor libraries. In this work, we present an open source system that, compared to existing approaches, achieves competitive computational speed while achieving higher portability. We achieve this by targeting the vendor-neutral OpenCL platform using a code-generation approach. We argue that our approach allows for both: (1) the rapid development of new computational kernels for existing hardware targets, and (2) the rapid tuning of existing computational kernels for new hardware targets. Results are presented for a case study of targeting the Qualcomm Snapdragon 820 mobile computing platform for CNN deployment.

==> SD820-op-eff-tab.full.tex <==
1 & 1 & 16 & $1\dx 28 \dx 28 \dx 192$ & conv  & 923us & 5.22GF/s & 2.37\\ 
1 & 1 & 16 & $5\dx 28 \dx 28 \dx 192$ & conv  & 3.80ms & 6.34GF/s & 2.88\\ 
1 & 1 & 16 & $20\dx 28 \dx 28 \dx 192$ & conv  & 14.9ms & 6.49GF/s & 2.95\\ 
1 & 1 & 16 & $1\dx 14 \dx 14 \dx 480$ & conv  & 956us & 3.15GF/s & 1.43\\ 
1 & 1 & 16 & $5\dx 14 \dx 14 \dx 480$ & conv  & 2.01ms & 7.48GF/s & 3.40\\ 
1 & 1 & 16 & $20\dx 14 \dx 14 \dx 480$ & conv  & 7.95ms & 7.58GF/s & 3.44\\ 
1 & 1 & 24 & $1\dx 14 \dx 14 \dx 512$ & conv  & 1.17ms & 4.10GF/s & 1.86\\ 
1 & 1 & 24 & $5\dx 14 \dx 14 \dx 512$ & conv  & 3.57ms & 6.75GF/s & 3.07\\ 
1 & 1 & 24 & $20\dx 14 \dx 14 \dx 512$ & conv  & 14.1ms & 6.86GF/s & 3.12\\ 
1 & 1 & 32 & $1\dx 28 \dx 28 \dx 192$ & conv  & 1.86ms & 5.17GF/s & 2.35\\ 
1 & 1 & 32 & $5\dx 28 \dx 28 \dx 192$ & conv  & 7.68ms & 6.27GF/s & 2.85\\ 
1 & 1 & 32 & $20\dx 28 \dx 28 \dx 192$ & conv  & 30.2ms & 6.38GF/s & 2.90\\ 
1 & 1 & 32 & $1\dx 28 \dx 28 \dx 256$ & conv  & 2.34ms & 5.48GF/s & 2.49\\ 
1 & 1 & 32 & $5\dx 28 \dx 28 \dx 256$ & conv  & 9.65ms & 6.66GF/s & 3.03\\ 
1 & 1 & 32 & $20\dx 28 \dx 28 \dx 256$ & conv  & 37.6ms & 6.83GF/s & 3.11\\ 
5 & 1 & 32 & $1\dx 28 \dx 28 \dx 16$ & conv  & 3.48ms & 5.76GF/s & 2.62\\ 
5 & 1 & 32 & $5\dx 28 \dx 28 \dx 16$ & conv  & 14.5ms & 6.93GF/s & 3.15\\ 
5 & 1 & 32 & $20\dx 28 \dx 28 \dx 16$ & conv  & 56.7ms & 7.08GF/s & 3.22\\ 
1 & 1 & 32 & $1\dx 14 \dx 14 \dx 512$ & conv  & 1.03ms & 6.22GF/s & 2.83\\ 
1 & 1 & 32 & $5\dx 14 \dx 14 \dx 512$ & conv  & 4.37ms & 7.35GF/s & 3.34\\ 
1 & 1 & 32 & $20\dx 14 \dx 14 \dx 512$ & conv  & 17.4ms & 7.38GF/s & 3.35\\ 
1 & 1 & 32 & $1\dx 14 \dx 14 \dx 528$ & conv  & 1.05ms & 6.33GF/s & 2.88\\ 
1 & 1 & 32 & $5\dx 14 \dx 14 \dx 528$ & conv  & 4.48ms & 7.40GF/s & 3.36\\ 
1 & 1 & 32 & $20\dx 14 \dx 14 \dx 528$ & conv  & 17.9ms & 7.38GF/s & 3.35\\ 
1 & 1 & 32 & $1\dx 7 \dx 7 \dx 832$ & conv  & 1.52ms & 1.72GF/s & 781m\\ 
1 & 1 & 32 & $5\dx 7 \dx 7 \dx 832$ & conv  & 1.65ms & 7.93GF/s & 3.60\\ 
1 & 1 & 32 & $20\dx 7 \dx 7 \dx 832$ & conv  & 6.53ms & 7.99GF/s & 3.63\\ 
5 & 1 & 48 & $1\dx 14 \dx 14 \dx 16$ & conv  & 1.93ms & 3.89GF/s & 1.77\\ 
5 & 1 & 48 & $5\dx 14 \dx 14 \dx 16$ & conv  & 6.93ms & 5.43GF/s & 2.47\\ 
5 & 1 & 48 & $20\dx 14 \dx 14 \dx 16$ & conv  & 25.2ms & 5.98GF/s & 2.72\\ 
1 & 1 & 48 & $1\dx 7 \dx 7 \dx 832$ & conv  & 1.73ms & 2.27GF/s & 1.03\\ 
1 & 1 & 48 & $5\dx 7 \dx 7 \dx 832$ & conv  & 3.52ms & 5.55GF/s & 2.52\\ 
1 & 1 & 48 & $20\dx 7 \dx 7 \dx 832$ & conv  & 12.3ms & 6.37GF/s & 2.90\\ 
1 & 1 & 64 & $1\dx 56 \dx 56 \dx 64$ & conv  & 6.22ms & 4.13GF/s & 1.88\\ 
1 & 1 & 64 & $5\dx 56 \dx 56 \dx 64$ & conv  & 30.8ms & 4.18GF/s & 1.90\\ 
1 & 1 & 64 & $20\dx 56 \dx 56 \dx 64$ & conv  & 123ms & 4.19GF/s & 1.90\\ 
7 & 2 & 64 & $1\dx 224 \dx 224 \dx 3$ & conv  & 42.4ms & 5.57GF/s & 2.53\\ 
7 & 2 & 64 & $5\dx 224 \dx 224 \dx 3$ & conv  & 212ms & 5.57GF/s & 2.53\\ 
7 & 2 & 64 & $20\dx 224 \dx 224 \dx 3$ & conv  & 848ms & 5.57GF/s & 2.53\\ 
1 & 1 & 64 & $1\dx 28 \dx 28 \dx 192$ & conv  & 3.31ms & 5.81GF/s & 2.64\\ 
1 & 1 & 64 & $5\dx 28 \dx 28 \dx 192$ & conv  & 15.2ms & 6.34GF/s & 2.88\\ 
1 & 1 & 64 & $20\dx 28 \dx 28 \dx 192$ & conv  & 60.2ms & 6.40GF/s & 2.91\\ 
1 & 1 & 64 & $1\dx 28 \dx 28 \dx 256$ & conv  & 4.17ms & 6.16GF/s & 2.80\\ 
1 & 1 & 64 & $5\dx 28 \dx 28 \dx 256$ & conv  & 19.0ms & 6.75GF/s & 3.07\\ 
1 & 1 & 64 & $20\dx 28 \dx 28 \dx 256$ & conv  & 74.9ms & 6.86GF/s & 3.12\\ 
1 & 1 & 64 & $1\dx 14 \dx 14 \dx 480$ & conv  & 2.08ms & 5.79GF/s & 2.63\\ 
1 & 1 & 64 & $5\dx 14 \dx 14 \dx 480$ & conv  & 8.14ms & 7.40GF/s & 3.36\\ 
1 & 1 & 64 & $20\dx 14 \dx 14 \dx 480$ & conv  & 31.8ms & 7.57GF/s & 3.44\\ 
1 & 1 & 64 & $1\dx 14 \dx 14 \dx 512$ & conv  & 2.14ms & 6.01GF/s & 2.73\\ 
1 & 1 & 64 & $5\dx 14 \dx 14 \dx 512$ & conv  & 8.84ms & 7.26GF/s & 3.30\\ 
1 & 1 & 64 & $20\dx 14 \dx 14 \dx 512$ & conv  & 33.8ms & 7.60GF/s & 3.45\\ 
5 & 1 & 64 & $1\dx 14 \dx 14 \dx 24$ & conv  & 2.64ms & 5.71GF/s & 2.59\\ 
5 & 1 & 64 & $5\dx 14 \dx 14 \dx 24$ & conv  & 10.9ms & 6.91GF/s & 3.14\\ 
5 & 1 & 64 & $20\dx 14 \dx 14 \dx 24$ & conv  & 42.5ms & 7.09GF/s & 3.22\\ 
5 & 1 & 64 & $1\dx 14 \dx 14 \dx 32$ & conv  & 3.46ms & 5.80GF/s & 2.64\\ 
5 & 1 & 64 & $5\dx 14 \dx 14 \dx 32$ & conv  & 14.2ms & 7.05GF/s & 3.20\\ 
5 & 1 & 64 & $20\dx 14 \dx 14 \dx 32$ & conv  & 55.3ms & 7.25GF/s & 3.30\\ 
1 & 1 & 96 & $1\dx 54 \dx 54 \dx 96$ & conv  & 13.9ms & 3.86GF/s & 1.76\\ 
1 & 1 & 96 & $5\dx 54 \dx 54 \dx 96$ & conv  & 69.6ms & 3.86GF/s & 1.76\\ 
1 & 1 & 96 & $20\dx 54 \dx 54 \dx 96$ & conv  & 277ms & 3.88GF/s & 1.76\\ 
1 & 1 & 96 & $1\dx 28 \dx 28 \dx 192$ & conv  & 6.27ms & 4.61GF/s & 2.09\\ 
1 & 1 & 96 & $5\dx 28 \dx 28 \dx 192$ & conv  & 30.3ms & 4.76GF/s & 2.16\\ 
1 & 1 & 96 & $20\dx 28 \dx 28 \dx 192$ & conv  & 120ms & 4.81GF/s & 2.19\\ 
11 & 4 & 96 & $1\dx 224 \dx 224 \dx 3$ & conv  & 40.4ms & 5.03GF/s & 2.29\\ 
11 & 4 & 96 & $1\dx 227 \dx 227 \dx 3$ & conv  & 42.3ms & 4.98GF/s & 2.26\\ 
11 & 4 & 96 & $5\dx 224 \dx 224 \dx 3$ & conv  & 201ms & 5.06GF/s & 2.30\\ 
11 & 4 & 96 & $5\dx 227 \dx 227 \dx 3$ & conv  & 209ms & 5.05GF/s & 2.29\\ 
11 & 4 & 96 & $20\dx 224 \dx 224 \dx 3$ & conv  & 802ms & 5.07GF/s & 2.30\\ 
11 & 4 & 96 & $20\dx 227 \dx 227 \dx 3$ & conv  & 834ms & 5.06GF/s & 2.30\\ 
1 & 1 & 96 & $1\dx 14 \dx 14 \dx 480$ & conv  & 4.09ms & 4.41GF/s & 2.01\\ 
1 & 1 & 96 & $5\dx 14 \dx 14 \dx 480$ & conv  & 16.5ms & 5.47GF/s & 2.49\\ 
1 & 1 & 96 & $20\dx 14 \dx 14 \dx 480$ & conv  & 64.7ms & 5.59GF/s & 2.54\\ 
5 & 1 & 96 & $1\dx 28 \dx 28 \dx 32$ & conv  & 22.7ms & 5.31GF/s & 2.41\\ 
5 & 1 & 96 & $5\dx 28 \dx 28 \dx 32$ & conv  & 109ms & 5.53GF/s & 2.51\\ 
5 & 1 & 96 & $20\dx 28 \dx 28 \dx 32$ & conv  & 431ms & 5.59GF/s & 2.54\\ 
1 & 1 & 112 & $1\dx 14 \dx 14 \dx 512$ & conv  & 4.31ms & 5.22GF/s & 2.37\\ 
1 & 1 & 112 & $5\dx 14 \dx 14 \dx 512$ & conv  & 17.6ms & 6.38GF/s & 2.90\\ 
1 & 1 & 112 & $20\dx 14 \dx 14 \dx 512$ & conv  & 67.6ms & 6.65GF/s & 3.02\\ 
1 & 1 & 128 & $1\dx 28 \dx 28 \dx 256$ & conv  & 7.99ms & 6.43GF/s & 2.92\\ 
1 & 1 & 128 & $5\dx 28 \dx 28 \dx 256$ & conv  & 38.4ms & 6.69GF/s & 3.04\\ 
1 & 1 & 128 & $20\dx 28 \dx 28 \dx 256$ & conv  & 151ms & 6.82GF/s & 3.10\\ 
1 & 1 & 128 & $1\dx 4 \dx 4 \dx 512$ & conv  & 709us & 2.96GF/s & 1.34\\ 
1 & 1 & 128 & $1\dx 14 \dx 14 \dx 512$ & conv  & 4.33ms & 5.93GF/s & 2.70\\ 
1 & 1 & 128 & $5\dx 4 \dx 4 \dx 512$ & conv  & 1.40ms & 7.49GF/s & 3.41\\ 
1 & 1 & 128 & $5\dx 14 \dx 14 \dx 512$ & conv  & 17.4ms & 7.40GF/s & 3.36\\ 
1 & 1 & 128 & $20\dx 4 \dx 4 \dx 512$ & conv  & 3.56ms & 11.8GF/s & 5.36\\ 
1 & 1 & 128 & $20\dx 14 \dx 14 \dx 512$ & conv  & 68.2ms & 7.54GF/s & 3.43\\ 
1 & 1 & 128 & $1\dx 4 \dx 4 \dx 528$ & conv  & 735us & 2.94GF/s & 1.34\\ 
1 & 1 & 128 & $1\dx 14 \dx 14 \dx 528$ & conv  & 4.39ms & 6.03GF/s & 2.74\\ 
1 & 1 & 128 & $5\dx 4 \dx 4 \dx 528$ & conv  & 1.50ms & 7.21GF/s & 3.28\\ 
1 & 1 & 128 & $5\dx 14 \dx 14 \dx 528$ & conv  & 18.1ms & 7.30GF/s & 3.32\\ 
1 & 1 & 128 & $20\dx 4 \dx 4 \dx 528$ & conv  & 3.75ms & 11.5GF/s & 5.24\\ 
1 & 1 & 128 & $20\dx 14 \dx 14 \dx 528$ & conv  & 70.3ms & 7.54GF/s & 3.43\\ 
5 & 1 & 128 & $1\dx 7 \dx 7 \dx 32$ & conv  & 1.78ms & 5.65GF/s & 2.57\\ 
5 & 1 & 128 & $1\dx 14 \dx 14 \dx 32$ & conv  & 6.90ms & 5.82GF/s & 2.65\\ 
5 & 1 & 128 & $5\dx 7 \dx 7 \dx 32$ & conv  & 7.13ms & 7.04GF/s & 3.20\\ 
5 & 1 & 128 & $5\dx 14 \dx 14 \dx 32$ & conv  & 28.4ms & 7.07GF/s & 3.21\\ 
5 & 1 & 128 & $20\dx 7 \dx 7 \dx 32$ & conv  & 28.3ms & 7.08GF/s & 3.22\\ 
5 & 1 & 128 & $20\dx 14 \dx 14 \dx 32$ & conv  & 110ms & 7.29GF/s & 3.31\\ 
1 & 1 & 128 & $1\dx 7 \dx 7 \dx 832$ & conv  & 1.67ms & 6.26GF/s & 2.85\\ 
1 & 1 & 128 & $5\dx 7 \dx 7 \dx 832$ & conv  & 6.78ms & 7.70GF/s & 3.50\\ 
1 & 1 & 128 & $20\dx 7 \dx 7 \dx 832$ & conv  & 27.1ms & 7.70GF/s & 3.50\\ 
3 & 1 & 128 & $1\dx 28 \dx 28 \dx 96$ & conv  & 25.3ms & 6.84GF/s & 3.11\\ 
3 & 1 & 128 & $5\dx 28 \dx 28 \dx 96$ & conv  & 121ms & 7.16GF/s & 3.25\\ 
3 & 1 & 128 & $20\dx 28 \dx 28 \dx 96$ & conv  & 479ms & 7.24GF/s & 3.29\\ 
5 & 1 & 128 & $1\dx 7 \dx 7 \dx 48$ & conv  & 2.60ms & 5.78GF/s & 2.63\\ 
5 & 1 & 128 & $5\dx 7 \dx 7 \dx 48$ & conv  & 10.4ms & 7.21GF/s & 3.28\\ 
5 & 1 & 128 & $20\dx 7 \dx 7 \dx 48$ & conv  & 41.4ms & 7.27GF/s & 3.31\\ 
1 & 1 & 144 & $1\dx 14 \dx 14 \dx 512$ & conv  & 6.28ms & 4.60GF/s & 2.09\\ 
1 & 1 & 144 & $5\dx 14 \dx 14 \dx 512$ & conv  & 25.3ms & 5.71GF/s & 2.60\\ 
1 & 1 & 144 & $20\dx 14 \dx 14 \dx 512$ & conv  & 99.1ms & 5.83GF/s & 2.65\\ 
1 & 1 & 160 & $1\dx 14 \dx 14 \dx 512$ & conv  & 6.28ms & 5.12GF/s & 2.33\\ 
1 & 1 & 160 & $5\dx 14 \dx 14 \dx 512$ & conv  & 25.6ms & 6.28GF/s & 2.85\\ 
1 & 1 & 160 & $20\dx 14 \dx 14 \dx 512$ & conv  & 102ms & 6.31GF/s & 2.87\\ 
1 & 1 & 160 & $1\dx 14 \dx 14 \dx 528$ & conv  & 6.64ms & 4.99GF/s & 2.27\\ 
1 & 1 & 160 & $5\dx 14 \dx 14 \dx 528$ & conv  & 26.8ms & 6.18GF/s & 2.81\\ 
1 & 1 & 160 & $20\dx 14 \dx 14 \dx 528$ & conv  & 103ms & 6.46GF/s & 2.94\\ 
1 & 1 & 160 & $1\dx 7 \dx 7 \dx 832$ & conv  & 3.23ms & 4.03GF/s & 1.83\\ 
1 & 1 & 160 & $5\dx 7 \dx 7 \dx 832$ & conv  & 9.85ms & 6.62GF/s & 3.01\\ 
1 & 1 & 160 & $20\dx 7 \dx 7 \dx 832$ & conv  & 40.0ms & 6.53GF/s & 2.97\\ 
1 & 1 & 192 & $1\dx 14 \dx 14 \dx 480$ & conv  & 6.06ms & 5.96GF/s & 2.71\\ 
1 & 1 & 192 & $5\dx 14 \dx 14 \dx 480$ & conv  & 24.3ms & 7.42GF/s & 3.37\\ 
1 & 1 & 192 & $20\dx 14 \dx 14 \dx 480$ & conv  & 94.7ms & 7.63GF/s & 3.47\\ 
3 & 1 & 192 & $1\dx 56 \dx 56 \dx 64$ & conv  & 100ms & 6.92GF/s & 3.14\\ 
3 & 1 & 192 & $5\dx 56 \dx 56 \dx 64$ & conv  & 499ms & 6.95GF/s & 3.16\\ 
3 & 1 & 192 & $20\dx 56 \dx 56 \dx 64$ & conv  & 1.99s & 6.96GF/s & 3.16\\ 
1 & 1 & 192 & $1\dx 7 \dx 7 \dx 832$ & conv  & 3.26ms & 4.81GF/s & 2.19\\ 
1 & 1 & 192 & $5\dx 7 \dx 7 \dx 832$ & conv  & 9.96ms & 7.86GF/s & 3.57\\ 
1 & 1 & 192 & $20\dx 7 \dx 7 \dx 832$ & conv  & 39.8ms & 7.87GF/s & 3.58\\ 
3 & 1 & 192 & $1\dx 28 \dx 28 \dx 128$ & conv  & 48.8ms & 7.11GF/s & 3.23\\ 
3 & 1 & 192 & $5\dx 28 \dx 28 \dx 128$ & conv  & 240ms & 7.22GF/s & 3.28\\ 
3 & 1 & 192 & $20\dx 28 \dx 28 \dx 128$ & conv  & 950ms & 7.30GF/s & 3.32\\ 
3 & 1 & 208 & $1\dx 14 \dx 14 \dx 96$ & conv  & 13.5ms & 5.22GF/s & 2.37\\ 
3 & 1 & 208 & $5\dx 14 \dx 14 \dx 96$ & conv  & 60.4ms & 5.84GF/s & 2.65\\ 
3 & 1 & 208 & $20\dx 14 \dx 14 \dx 96$ & conv  & 240ms & 5.87GF/s & 2.67\\ 
3 & 1 & 224 & $1\dx 14 \dx 14 \dx 112$ & conv  & 15.6ms & 5.67GF/s & 2.58\\ 
3 & 1 & 224 & $5\dx 14 \dx 14 \dx 112$ & conv  & 70.0ms & 6.32GF/s & 2.87\\ 
3 & 1 & 224 & $20\dx 14 \dx 14 \dx 112$ & conv  & 278ms & 6.36GF/s & 2.89\\ 
1 & 1 & 256 & $1\dx 27 \dx 27 \dx 256$ & conv  & 13.9ms & 6.86GF/s & 3.12\\ 
1 & 1 & 256 & $5\dx 27 \dx 27 \dx 256$ & conv  & 69.2ms & 6.90GF/s & 3.14\\ 
1 & 1 & 256 & $20\dx 27 \dx 27 \dx 256$ & conv  & 274ms & 6.97GF/s & 3.17\\ 
1 & 1 & 256 & $1\dx 14 \dx 14 \dx 528$ & conv  & 7.80ms & 6.80GF/s & 3.09\\ 
1 & 1 & 256 & $5\dx 14 \dx 14 \dx 528$ & conv  & 34.9ms & 7.59GF/s & 3.45\\ 
1 & 1 & 256 & $20\dx 14 \dx 14 \dx 528$ & conv  & 138ms & 7.66GF/s & 3.48\\ 
1 & 1 & 256 & $1\dx 7 \dx 7 \dx 832$ & conv  & 3.32ms & 6.28GF/s & 2.85\\ 
1 & 1 & 256 & $5\dx 7 \dx 7 \dx 832$ & conv  & 13.6ms & 7.70GF/s & 3.50\\ 
1 & 1 & 256 & $20\dx 7 \dx 7 \dx 832$ & conv  & 52.7ms & 7.92GF/s & 3.60\\ 
3 & 1 & 256 & $1\dx 14 \dx 14 \dx 128$ & conv  & 17.7ms & 6.52GF/s & 2.96\\ 
3 & 1 & 256 & $5\dx 14 \dx 14 \dx 128$ & conv  & 79.5ms & 7.27GF/s & 3.31\\ 
3 & 1 & 256 & $20\dx 14 \dx 14 \dx 128$ & conv  & 315ms & 7.34GF/s & 3.33\\ 
5 & 1 & 256 & $1\dx 27 \dx 27 \dx 96$ & conv  & 119ms & 7.55GF/s & 3.43\\ 
5 & 1 & 256 & $5\dx 27 \dx 27 \dx 96$ & conv  & 589ms & 7.60GF/s & 3.45\\ 
5 & 1 & 256 & $20\dx 27 \dx 27 \dx 96$ & conv  & 2.36s & 7.60GF/s & 3.46\\ 
3 & 1 & 256 & $1\dx 13 \dx 13 \dx 384$ & conv  & 44.0ms & 6.79GF/s & 3.09\\ 
3 & 1 & 256 & $5\dx 13 \dx 13 \dx 384$ & conv  & 200ms & 7.47GF/s & 3.39\\ 
3 & 1 & 256 & $20\dx 13 \dx 13 \dx 384$ & conv  & 788ms & 7.59GF/s & 3.45\\ 
3 & 1 & 288 & $1\dx 14 \dx 14 \dx 144$ & conv  & 25.1ms & 5.83GF/s & 2.65\\ 
3 & 1 & 288 & $5\dx 14 \dx 14 \dx 144$ & conv  & 111ms & 6.61GF/s & 3.01\\ 
3 & 1 & 288 & $20\dx 14 \dx 14 \dx 144$ & conv  & 437ms & 6.70GF/s & 3.04\\ 
3 & 1 & 320 & $1\dx 7 \dx 7 \dx 160$ & conv  & 9.25ms & 4.88GF/s & 2.22\\ 
3 & 1 & 320 & $1\dx 14 \dx 14 \dx 160$ & conv  & 27.8ms & 6.49GF/s & 2.95\\ 
3 & 1 & 320 & $5\dx 7 \dx 7 \dx 160$ & conv  & 31.2ms & 7.24GF/s & 3.29\\ 
3 & 1 & 320 & $5\dx 14 \dx 14 \dx 160$ & conv  & 123ms & 7.37GF/s & 3.35\\ 
3 & 1 & 320 & $20\dx 7 \dx 7 \dx 160$ & conv  & 122ms & 7.41GF/s & 3.37\\ 
3 & 1 & 320 & $20\dx 14 \dx 14 \dx 160$ & conv  & 484ms & 7.46GF/s & 3.39\\ 
1 & 1 & 384 & $1\dx 13 \dx 13 \dx 384$ & conv  & 7.48ms & 6.66GF/s & 3.03\\ 
1 & 1 & 384 & $5\dx 13 \dx 13 \dx 384$ & conv  & 34.7ms & 7.18GF/s & 3.27\\ 
1 & 1 & 384 & $20\dx 13 \dx 13 \dx 384$ & conv  & 133ms & 7.47GF/s & 3.39\\ 
1 & 1 & 384 & $1\dx 7 \dx 7 \dx 832$ & conv  & 4.93ms & 6.36GF/s & 2.89\\ 
1 & 1 & 384 & $5\dx 7 \dx 7 \dx 832$ & conv  & 20.0ms & 7.83GF/s & 3.56\\ 
1 & 1 & 384 & $20\dx 7 \dx 7 \dx 832$ & conv  & 78.4ms & 7.99GF/s & 3.63\\ 
3 & 1 & 384 & $1\dx 7 \dx 7 \dx 192$ & conv  & 11.1ms & 5.84GF/s & 2.65\\ 
3 & 1 & 384 & $5\dx 7 \dx 7 \dx 192$ & conv  & 44.7ms & 7.27GF/s & 3.30\\ 
3 & 1 & 384 & $20\dx 7 \dx 7 \dx 192$ & conv  & 176ms & 7.40GF/s & 3.37\\ 
3 & 1 & 384 & $1\dx 13 \dx 13 \dx 256$ & conv  & 44.4ms & 6.74GF/s & 3.06\\ 
3 & 1 & 384 & $5\dx 13 \dx 13 \dx 256$ & conv  & 204ms & 7.33GF/s & 3.33\\ 
3 & 1 & 384 & $20\dx 13 \dx 13 \dx 256$ & conv  & 794ms & 7.53GF/s & 3.42\\ 
3 & 1 & 384 & $1\dx 13 \dx 13 \dx 384$ & conv  & 66.4ms & 6.75GF/s & 3.07\\ 
3 & 1 & 384 & $5\dx 13 \dx 13 \dx 384$ & conv  & 305ms & 7.36GF/s & 3.34\\ 
3 & 1 & 384 & $20\dx 13 \dx 13 \dx 384$ & conv  & 1.19s & 7.56GF/s & 3.44\\ 
1 & 1 & 1000 & $1\dx 1 \dx 1 \dx 1024$ & conv  & 24.4ms & 84.0MF/s & 38.2m\\ 
1 & 1 & 1000 & $1\dx 6 \dx 6 \dx 1024$ & conv  & 16.1ms & 4.57GF/s & 2.08\\ 
1 & 1 & 1000 & $5\dx 1 \dx 1 \dx 1024$ & conv  & 6.01ms & 1.70GF/s & 774m\\ 
1 & 1 & 1000 & $5\dx 6 \dx 6 \dx 1024$ & conv  & 48.7ms & 7.56GF/s & 3.44\\ 
1 & 1 & 1000 & $20\dx 1 \dx 1 \dx 1024$ & conv  & 6.25ms & 6.55GF/s & 2.98\\ 
1 & 1 & 1000 & $20\dx 6 \dx 6 \dx 1024$ & conv  & 187ms & 7.89GF/s & 3.59\\ 
1 & 1 & 1000 & $1\dx 1 \dx 1 \dx 4096$ & conv  & 95.9ms & 85.4MF/s & 38.8m\\ 
1 & 1 & 1000 & $5\dx 1 \dx 1 \dx 4096$ & conv  & 24.7ms & 1.66GF/s & 754m\\ 
1 & 1 & 1000 & $20\dx 1 \dx 1 \dx 4096$ & conv  & 39.6ms & 4.13GF/s & 1.88\\ 
1 & 1 & 1024 & $1\dx 6 \dx 6 \dx 1024$ & conv  & 16.1ms & 4.69GF/s & 2.13\\ 
1 & 1 & 1024 & $5\dx 6 \dx 6 \dx 1024$ & conv  & 48.8ms & 7.73GF/s & 3.51\\ 
1 & 1 & 1024 & $20\dx 6 \dx 6 \dx 1024$ & conv  & 187ms & 8.09GF/s & 3.68\\ 
4 & 1 & 1024 & $1\dx 4 \dx 4 \dx 128$ & conv  & 56.1ms & 74.7MF/s & 34.0m\\ 
4 & 1 & 1024 & $5\dx 4 \dx 4 \dx 128$ & conv  & 13.4ms & 1.57GF/s & 713m\\ 
4 & 1 & 1024 & $20\dx 4 \dx 4 \dx 128$ & conv  & 18.6ms & 4.51GF/s & 2.05\\ 
3 & 1 & 1024 & $1\dx 6 \dx 6 \dx 384$ & conv  & 57.6ms & 4.42GF/s & 2.01\\ 
3 & 1 & 1024 & $5\dx 6 \dx 6 \dx 384$ & conv  & 180ms & 7.07GF/s & 3.22\\ 
3 & 1 & 1024 & $20\dx 6 \dx 6 \dx 384$ & conv  & 690ms & 7.38GF/s & 3.35\\ 
1 & 1 & 4096 & $1\dx 1 \dx 1 \dx 4096$ & conv  & 395ms & 85.0MF/s & 38.6m\\ 
1 & 1 & 4096 & $5\dx 1 \dx 1 \dx 4096$ & conv  & 94.2ms & 1.78GF/s & 809m\\ 
1 & 1 & 4096 & $20\dx 1 \dx 1 \dx 4096$ & conv  & 140ms & 4.79GF/s & 2.18\\ 
6 & 1 & 4096 & $1\dx 6 \dx 6 \dx 256$ & conv  & 1.37s & 54.9MF/s & 25.0m\\ 
6 & 1 & 4096 & $5\dx 6 \dx 6 \dx 256$ & conv  & 312ms & 1.21GF/s & 550m\\ 
6 & 1 & 4096 & $20\dx 6 \dx 6 \dx 256$ & conv  & 284ms & 5.32GF/s & 2.42\\ 


==> SD820-op-eff-tab.tex <==
1 & 1 & 256 & $20\dx 13 \dx 13 \dx 256$ & conv  & 62.1ms & 7.14GF/s & 3.24\\ 
3 & 1 & 256 & $20\dx 13 \dx 13 \dx 128$ & conv  & 268ms & 14.9GF/s & 6.76\\ 
7 & 2 & 96 & $20\dx 205 \dx 205 \dx 3$ & conv  & 1.27s & 4.43GF/s & 2.02\\ 


==> SD820-op-info-tab.tex <==
1 & 1 & 256 & 20 & $13 \dx 13 \dx 256$ & $13 \dx 13 \dx 256$ & 7.19MB & 443MF & 61.7 & $3380 \dx 256 \dx 256$\\ 
3 & 1 & 256 & 20 & $13 \dx 13 \dx 128$ & $13 \dx 13 \dx 256$ & 7.55MB & 3.99GF & 528 & $3380 \dx 2304 \dx 256$\\ 
7 & 2 & 96 & 20 & $205 \dx 205 \dx 3$ & $100 \dx 100 \dx 96$ & 86.9MB & 5.64GF & 64.9 & $200000 \dx 147 \dx 96$\\ 


==> cnn-SD820-boda-eff-tab.tex <==
1 & 1 & 96 & $20\dx 55 \dx 55 \dx 96$ & \verb|k1conv_simd| & 26.2ms & 42.5GF/s & 16.6\\ 
11 & 4 & 96 & $20\dx 227 \dx 227 \dx 3$ & \verb|conv_simd| & 120ms & 35.1GF/s & 13.7\\ 
1 & 1 & 256 & $20\dx 27 \dx 27 \dx 256$ & \verb|k1conv_simd| & 36.2ms & 52.7GF/s & 20.6\\ 
5 & 1 & 256 & $20\dx 27 \dx 27 \dx 96$ & \verb|conv_simd| & 504ms & 35.6GF/s & 13.9\\ 
1 & 1 & 384 & $20\dx 13 \dx 13 \dx 384$ & \verb|k1conv_simd| & 16.0ms & 62.2GF/s & 24.3\\ 
3 & 1 & 384 & $20\dx 13 \dx 13 \dx 256$ & \verb|conv_simd| & 320ms & 18.7GF/s & 7.30\\ 
1 & 1 & 1000 & $20\dx 6 \dx 6 \dx 1024$ & \verb|k1conv_simd| & 20.6ms & 71.5GF/s & 27.9\\ 
1 & 1 & 1024 & $20\dx 6 \dx 6 \dx 1024$ & \verb|k1conv_simd| & 20.5ms & 73.7GF/s & 28.8\\ 
3 & 1 & 1024 & $20\dx 6 \dx 6 \dx 384$ & \verb|conv_simd| & 209ms & 24.4GF/s & 9.52\\ 


==> cnn-titanX-boda-eff-tab.tex <==
1 & 1 & 96 & $20\dx 55 \dx 55 \dx 96$ & \verb|k1conv| & 778us & 1.43TF/s & 21.7\\ 
11 & 4 & 96 & $20\dx 227 \dx 227 \dx 3$ & \verb|tconv| & 1.46ms & 2.89TF/s & 43.8\\ 
1 & 1 & 256 & $20\dx 27 \dx 27 \dx 256$ & \verb|k1conv| & 786us & 2.43TF/s & 36.8\\ 
5 & 1 & 256 & $20\dx 27 \dx 27 \dx 96$ & \verb|tconv| & 5.42ms & 3.30TF/s & 50.0\\ 
1 & 1 & 384 & $20\dx 13 \dx 13 \dx 384$ & \verb|k1conv| & 391us & 2.55TF/s & 38.6\\ 
3 & 1 & 384 & $20\dx 13 \dx 13 \dx 256$ & \verb|tconv| & 2.94ms & 2.04TF/s & 30.8\\ 
1 & 1 & 1000 & $20\dx 6 \dx 6 \dx 1024$ & \verb|k1conv| & 437us & 3.37TF/s & 51.1\\ 
1 & 1 & 1024 & $20\dx 6 \dx 6 \dx 1024$ & \verb|k1conv| & 438us & 3.45TF/s & 52.2\\ 
3 & 1 & 1024 & $20\dx 6 \dx 6 \dx 384$ & \verb|tconv| & 1.66ms & 3.06TF/s & 46.4\\ 


==> cnn-titanX-cudnn-eff-tab.tex <==
1 & 1 & 96 & $20\dx 55 \dx 55 \dx 96$ & \verb|cudnn_conv| & 902us & 1.24TF/s & 18.7\\ 
11 & 4 & 96 & $20\dx 227 \dx 227 \dx 3$ & \verb|cudnn_conv| & 1.61ms & 2.61TF/s & 39.6\\ 
1 & 1 & 256 & $20\dx 27 \dx 27 \dx 256$ & \verb|cudnn_conv| & 761us & 2.51TF/s & 38.0\\ 
5 & 1 & 256 & $20\dx 27 \dx 27 \dx 96$ & \verb|cudnn_conv| & 4.08ms & 4.39TF/s & 66.5\\ 
1 & 1 & 384 & $20\dx 13 \dx 13 \dx 384$ & \verb|cudnn_conv| & 429us & 2.32TF/s & 35.2\\ 
3 & 1 & 384 & $20\dx 13 \dx 13 \dx 256$ & \verb|cudnn_conv| & 1.62ms & 3.70TF/s & 56.0\\ 
1 & 1 & 1000 & $20\dx 6 \dx 6 \dx 1024$ & \verb|cudnn_conv| & 1.14ms & 1.30TF/s & 19.7\\ 
1 & 1 & 1024 & $20\dx 6 \dx 6 \dx 1024$ & \verb|cudnn_conv| & 896us & 1.69TF/s & 25.5\\ 
3 & 1 & 1024 & $20\dx 6 \dx 6 \dx 384$ & \verb|cudnn_conv| & 1.20ms & 4.24TF/s & 64.2\\ 


==> op-eff-tab.full.tex <==
1 & 1 & 16 & $1\dx 28 \dx 28 \dx 192$ & conv  & 341us & 14.1GF/s & 214m\\ 
1 & 1 & 16 & $1\dx 28 \dx 28 \dx 192$ & tconv  & 201us & 24.0GF/s & 364m\\ 
1 & 1 & 16 & $5\dx 28 \dx 28 \dx 192$ & conv  & 396us & 60.8GF/s & 921m\\ 
1 & 1 & 16 & $5\dx 28 \dx 28 \dx 192$ & tconv  & 253us & 95.2GF/s & 1.44\\ 
1 & 1 & 16 & $20\dx 28 \dx 28 \dx 192$ & conv  & 479us & 201GF/s & 3.05\\ 
1 & 1 & 16 & $20\dx 28 \dx 28 \dx 192$ & tconv  & 294us & 328GF/s & 4.97\\ 
1 & 1 & 16 & $1\dx 14 \dx 14 \dx 480$ & conv  & 781us & 3.85GF/s & 58.4m\\ 
1 & 1 & 16 & $1\dx 14 \dx 14 \dx 480$ & tconv  & 454us & 6.64GF/s & 101m\\ 
1 & 1 & 16 & $5\dx 14 \dx 14 \dx 480$ & conv  & 791us & 19.0GF/s & 288m\\ 
1 & 1 & 16 & $5\dx 14 \dx 14 \dx 480$ & tconv  & 570us & 26.4GF/s & 400m\\ 
1 & 1 & 16 & $20\dx 14 \dx 14 \dx 480$ & conv  & 1.05ms & 57.3GF/s & 868m\\ 
1 & 1 & 16 & $20\dx 14 \dx 14 \dx 480$ & tconv  & 599us & 100GF/s & 1.52\\ 
1 & 1 & 24 & $1\dx 14 \dx 14 \dx 512$ & conv  & 695us & 6.93GF/s & 105m\\ 
1 & 1 & 24 & $1\dx 14 \dx 14 \dx 512$ & tconv  & 495us & 9.74GF/s & 148m\\ 
1 & 1 & 24 & $5\dx 14 \dx 14 \dx 512$ & conv  & 704us & 34.2GF/s & 519m\\ 
1 & 1 & 24 & $5\dx 14 \dx 14 \dx 512$ & tconv  & 520us & 46.3GF/s & 702m\\ 
1 & 1 & 24 & $20\dx 14 \dx 14 \dx 512$ & conv  & 915us & 105GF/s & 1.59\\ 
1 & 1 & 24 & $20\dx 14 \dx 14 \dx 512$ & tconv  & 633us & 152GF/s & 2.31\\ 
1 & 1 & 32 & $1\dx 28 \dx 28 \dx 192$ & conv  & 229us & 42.2GF/s & 639m\\ 
1 & 1 & 32 & $1\dx 28 \dx 28 \dx 192$ & tconv  & 202us & 47.7GF/s & 723m\\ 
1 & 1 & 32 & $5\dx 28 \dx 28 \dx 192$ & conv  & 282us & 171GF/s & 2.59\\ 
1 & 1 & 32 & $5\dx 28 \dx 28 \dx 192$ & tconv  & 238us & 203GF/s & 3.07\\ 
1 & 1 & 32 & $20\dx 28 \dx 28 \dx 192$ & conv  & 343us & 562GF/s & 8.52\\ 
1 & 1 & 32 & $20\dx 28 \dx 28 \dx 192$ & tconv  & 320us & 601GF/s & 9.11\\ 
1 & 1 & 32 & $1\dx 28 \dx 28 \dx 256$ & conv  & 297us & 43.3GF/s & 655m\\ 
1 & 1 & 32 & $1\dx 28 \dx 28 \dx 256$ & tconv  & 259us & 49.6GF/s & 751m\\ 
1 & 1 & 32 & $5\dx 28 \dx 28 \dx 256$ & conv  & 368us & 174GF/s & 2.64\\ 
1 & 1 & 32 & $5\dx 28 \dx 28 \dx 256$ & tconv  & 311us & 206GF/s & 3.13\\ 
1 & 1 & 32 & $20\dx 28 \dx 28 \dx 256$ & conv  & 436us & 589GF/s & 8.92\\ 
1 & 1 & 32 & $20\dx 28 \dx 28 \dx 256$ & tconv  & 407us & 631GF/s & 9.57\\ 
5 & 1 & 32 & $1\dx 28 \dx 28 \dx 16$ & conv  & 521us & 38.5GF/s & 584m\\ 
5 & 1 & 32 & $1\dx 28 \dx 28 \dx 16$ & tconv  & 106us & 189GF/s & 2.86\\ 
5 & 1 & 32 & $5\dx 28 \dx 28 \dx 16$ & conv  & 522us & 192GF/s & 2.91\\ 
5 & 1 & 32 & $5\dx 28 \dx 28 \dx 16$ & tconv  & 111us & 907GF/s & 13.7\\ 
5 & 1 & 32 & $20\dx 28 \dx 28 \dx 16$ & conv  & 586us & 685GF/s & 10.4\\ 
5 & 1 & 32 & $20\dx 28 \dx 28 \dx 16$ & tconv  & 194us & 2.07TF/s & 31.4\\ 
1 & 1 & 32 & $1\dx 14 \dx 14 \dx 512$ & conv  & 553us & 11.6GF/s & 176m\\ 
1 & 1 & 32 & $1\dx 14 \dx 14 \dx 512$ & tconv  & 471us & 13.6GF/s & 206m\\ 
1 & 1 & 32 & $5\dx 14 \dx 14 \dx 512$ & conv  & 567us & 56.6GF/s & 857m\\ 
1 & 1 & 32 & $5\dx 14 \dx 14 \dx 512$ & tconv  & 552us & 58.2GF/s & 882m\\ 
1 & 1 & 32 & $20\dx 14 \dx 14 \dx 512$ & conv  & 707us & 182GF/s & 2.75\\ 
1 & 1 & 32 & $20\dx 14 \dx 14 \dx 512$ & tconv  & 610us & 210GF/s & 3.19\\ 
1 & 1 & 32 & $1\dx 14 \dx 14 \dx 528$ & conv  & 570us & 11.6GF/s & 176m\\ 
1 & 1 & 32 & $1\dx 14 \dx 14 \dx 528$ & tconv  & 499us & 13.3GF/s & 201m\\ 
1 & 1 & 32 & $5\dx 14 \dx 14 \dx 528$ & conv  & 583us & 56.8GF/s & 860m\\ 
1 & 1 & 32 & $5\dx 14 \dx 14 \dx 528$ & tconv  & 594us & 55.8GF/s & 845m\\ 
1 & 1 & 32 & $20\dx 14 \dx 14 \dx 528$ & conv  & 730us & 182GF/s & 2.75\\ 
1 & 1 & 32 & $20\dx 14 \dx 14 \dx 528$ & tconv  & 637us & 208GF/s & 3.15\\ 
1 & 1 & 32 & $1\dx 7 \dx 7 \dx 832$ & conv  & 846us & 3.08GF/s & 46.7m\\ 
1 & 1 & 32 & $1\dx 7 \dx 7 \dx 832$ & tconv  & 730us & 3.57GF/s & 54.1m\\ 
1 & 1 & 32 & $5\dx 7 \dx 7 \dx 832$ & conv  & 892us & 14.6GF/s & 222m\\ 
1 & 1 & 32 & $5\dx 7 \dx 7 \dx 832$ & tconv  & 782us & 16.7GF/s & 253m\\ 
1 & 1 & 32 & $20\dx 7 \dx 7 \dx 832$ & conv  & 1.10ms & 47.5GF/s & 720m\\ 
1 & 1 & 32 & $20\dx 7 \dx 7 \dx 832$ & tconv  & 915us & 57.0GF/s & 864m\\ 
5 & 1 & 48 & $1\dx 14 \dx 14 \dx 16$ & conv  & 521us & 14.4GF/s & 219m\\ 
5 & 1 & 48 & $1\dx 14 \dx 14 \dx 16$ & tconv  & 99.6us & 75.5GF/s & 1.14\\ 
5 & 1 & 48 & $5\dx 14 \dx 14 \dx 16$ & conv  & 523us & 71.9GF/s & 1.09\\ 
5 & 1 & 48 & $5\dx 14 \dx 14 \dx 16$ & tconv  & 107us & 353GF/s & 5.35\\ 
5 & 1 & 48 & $20\dx 14 \dx 14 \dx 16$ & conv  & 526us & 286GF/s & 4.33\\ 
5 & 1 & 48 & $20\dx 14 \dx 14 \dx 16$ & tconv  & 141us & 1.07TF/s & 16.1\\ 
1 & 1 & 48 & $1\dx 7 \dx 7 \dx 832$ & conv  & 835us & 4.69GF/s & 71.0m\\ 
1 & 1 & 48 & $1\dx 7 \dx 7 \dx 832$ & tconv  & 733us & 5.34GF/s & 80.9m\\ 
1 & 1 & 48 & $5\dx 7 \dx 7 \dx 832$ & conv  & 941us & 20.8GF/s & 315m\\ 
1 & 1 & 48 & $5\dx 7 \dx 7 \dx 832$ & tconv  & 772us & 25.3GF/s & 384m\\ 
1 & 1 & 48 & $20\dx 7 \dx 7 \dx 832$ & conv  & 1.10ms & 71.4GF/s & 1.08\\ 
1 & 1 & 48 & $20\dx 7 \dx 7 \dx 832$ & tconv  & 909us & 86.2GF/s & 1.31\\ 
1 & 1 & 64 & $1\dx 56 \dx 56 \dx 64$ & conv  & 85.9us & 299GF/s & 4.53\\ 
1 & 1 & 64 & $1\dx 56 \dx 56 \dx 64$ & k1conv  & 50.1us & 512GF/s & 7.76\\ 
1 & 1 & 64 & $5\dx 56 \dx 56 \dx 64$ & conv  & 300us & 428GF/s & 6.49\\ 
1 & 1 & 64 & $5\dx 56 \dx 56 \dx 64$ & k1conv  & 149us & 860GF/s & 13.0\\ 
1 & 1 & 64 & $20\dx 56 \dx 56 \dx 64$ & conv  & 830us & 619GF/s & 9.38\\ 
1 & 1 & 64 & $20\dx 56 \dx 56 \dx 64$ & k1conv  & 424us & 1.21TF/s & 18.4\\ 
7 & 2 & 64 & $1\dx 224 \dx 224 \dx 3$ & conv  & 274us & 860GF/s & 13.0\\ 
7 & 2 & 64 & $1\dx 224 \dx 224 \dx 3$ & tconv  & 167us & 1.41TF/s & 21.4\\ 
7 & 2 & 64 & $5\dx 224 \dx 224 \dx 3$ & conv  & 1.14ms & 1.03TF/s & 15.7\\ 
7 & 2 & 64 & $5\dx 224 \dx 224 \dx 3$ & tconv  & 604us & 1.95TF/s & 29.6\\ 
7 & 2 & 64 & $20\dx 224 \dx 224 \dx 3$ & conv  & 3.99ms & 1.18TF/s & 17.9\\ 
7 & 2 & 64 & $20\dx 224 \dx 224 \dx 3$ & tconv  & 2.21ms & 2.14TF/s & 32.4\\ 
1 & 1 & 64 & $1\dx 28 \dx 28 \dx 192$ & conv  & 169us & 114GF/s & 1.73\\ 
1 & 1 & 64 & $1\dx 28 \dx 28 \dx 192$ & k1conv  & 59.4us & 324GF/s & 4.91\\ 
1 & 1 & 64 & $5\dx 28 \dx 28 \dx 192$ & conv  & 222us & 433GF/s & 6.57\\ 
1 & 1 & 64 & $5\dx 28 \dx 28 \dx 192$ & k1conv  & 90.4us & 1.07TF/s & 16.2\\ 
1 & 1 & 64 & $20\dx 28 \dx 28 \dx 192$ & conv  & 568us & 678GF/s & 10.3\\ 
1 & 1 & 64 & $20\dx 28 \dx 28 \dx 192$ & k1conv  & 209us & 1.84TF/s & 28.0\\ 
1 & 1 & 64 & $1\dx 28 \dx 28 \dx 256$ & conv  & 217us & 118GF/s & 1.79\\ 
1 & 1 & 64 & $1\dx 28 \dx 28 \dx 256$ & k1conv  & 70.3us & 365GF/s & 5.54\\ 
1 & 1 & 64 & $5\dx 28 \dx 28 \dx 256$ & conv  & 289us & 445GF/s & 6.74\\ 
1 & 1 & 64 & $5\dx 28 \dx 28 \dx 256$ & k1conv  & 107us & 1.21TF/s & 18.3\\ 
1 & 1 & 64 & $20\dx 28 \dx 28 \dx 256$ & conv  & 707us & 727GF/s & 11.0\\ 
1 & 1 & 64 & $20\dx 28 \dx 28 \dx 256$ & k1conv  & 245us & 2.10TF/s & 31.8\\ 
1 & 1 & 64 & $1\dx 14 \dx 14 \dx 480$ & conv  & 387us & 31.1GF/s & 472m\\ 
1 & 1 & 64 & $1\dx 14 \dx 14 \dx 480$ & k1conv  & 121us & 99.5GF/s & 1.51\\ 
1 & 1 & 64 & $5\dx 14 \dx 14 \dx 480$ & conv  & 388us & 155GF/s & 2.35\\ 
1 & 1 & 64 & $5\dx 14 \dx 14 \dx 480$ & k1conv  & 110us & 550GF/s & 8.33\\ 
1 & 1 & 64 & $20\dx 14 \dx 14 \dx 480$ & conv  & 518us & 465GF/s & 7.04\\ 
1 & 1 & 64 & $20\dx 14 \dx 14 \dx 480$ & k1conv  & 167us & 1.44TF/s & 21.9\\ 
1 & 1 & 64 & $1\dx 14 \dx 14 \dx 512$ & conv  & 411us & 31.3GF/s & 474m\\ 
1 & 1 & 64 & $1\dx 14 \dx 14 \dx 512$ & k1conv  & 114us & 113GF/s & 1.71\\ 
1 & 1 & 64 & $5\dx 14 \dx 14 \dx 512$ & conv  & 412us & 156GF/s & 2.36\\ 
1 & 1 & 64 & $5\dx 14 \dx 14 \dx 512$ & k1conv  & 115us & 560GF/s & 8.48\\ 
1 & 1 & 64 & $20\dx 14 \dx 14 \dx 512$ & conv  & 551us & 466GF/s & 7.07\\ 
1 & 1 & 64 & $20\dx 14 \dx 14 \dx 512$ & k1conv  & 172us & 1.49TF/s & 22.6\\ 
5 & 1 & 64 & $1\dx 14 \dx 14 \dx 24$ & conv  & 596us & 25.3GF/s & 383m\\ 
5 & 1 & 64 & $1\dx 14 \dx 14 \dx 24$ & tconv  & 143us & 105GF/s & 1.59\\ 
5 & 1 & 64 & $5\dx 14 \dx 14 \dx 24$ & conv  & 598us & 126GF/s & 1.91\\ 
5 & 1 & 64 & $5\dx 14 \dx 14 \dx 24$ & tconv  & 146us & 514GF/s & 7.79\\ 
5 & 1 & 64 & $20\dx 14 \dx 14 \dx 24$ & conv  & 663us & 454GF/s & 6.88\\ 
5 & 1 & 64 & $20\dx 14 \dx 14 \dx 24$ & tconv  & 189us & 1.59TF/s & 24.1\\ 
5 & 1 & 64 & $1\dx 14 \dx 14 \dx 32$ & conv  & 785us & 25.6GF/s & 388m\\ 
5 & 1 & 64 & $1\dx 14 \dx 14 \dx 32$ & tconv  & 182us & 110GF/s & 1.67\\ 
5 & 1 & 64 & $5\dx 14 \dx 14 \dx 32$ & conv  & 788us & 127GF/s & 1.93\\ 
5 & 1 & 64 & $5\dx 14 \dx 14 \dx 32$ & tconv  & 539us & 186GF/s & 2.82\\ 
5 & 1 & 64 & $20\dx 14 \dx 14 \dx 32$ & conv  & 819us & 490GF/s & 7.42\\ 
5 & 1 & 64 & $20\dx 14 \dx 14 \dx 32$ & tconv  & 239us & 1.68TF/s & 25.4\\ 
1 & 1 & 96 & $1\dx 54 \dx 54 \dx 96$ & conv  & 124us & 435GF/s & 6.59\\ 
1 & 1 & 96 & $1\dx 54 \dx 54 \dx 96$ & k1conv  & 70.8us & 759GF/s & 11.5\\ 
1 & 1 & 96 & $5\dx 54 \dx 54 \dx 96$ & conv  & 456us & 590GF/s & 8.94\\ 
1 & 1 & 96 & $5\dx 54 \dx 54 \dx 96$ & k1conv  & 231us & 1.16TF/s & 17.6\\ 
1 & 1 & 96 & $20\dx 54 \dx 54 \dx 96$ & conv  & 1.50ms & 715GF/s & 10.8\\ 
1 & 1 & 96 & $20\dx 54 \dx 54 \dx 96$ & k1conv  & 771us & 1.39TF/s & 21.1\\ 
1 & 1 & 96 & $1\dx 28 \dx 28 \dx 192$ & conv  & 171us & 169GF/s & 2.56\\ 
1 & 1 & 96 & $1\dx 28 \dx 28 \dx 192$ & k1conv  & 65.1us & 444GF/s & 6.73\\ 
1 & 1 & 96 & $5\dx 28 \dx 28 \dx 192$ & conv  & 255us & 567GF/s & 8.59\\ 
1 & 1 & 96 & $5\dx 28 \dx 28 \dx 192$ & k1conv  & 123us & 1.18TF/s & 17.8\\ 
1 & 1 & 96 & $20\dx 28 \dx 28 \dx 192$ & conv  & 668us & 865GF/s & 13.1\\ 
1 & 1 & 96 & $20\dx 28 \dx 28 \dx 192$ & k1conv  & 334us & 1.73TF/s & 26.2\\ 
11 & 4 & 96 & $1\dx 224 \dx 224 \dx 3$ & conv  & 429us & 474GF/s & 7.18\\ 
11 & 4 & 96 & $1\dx 224 \dx 224 \dx 3$ & tconv  & 151us & 1.35TF/s & 20.5\\ 
11 & 4 & 96 & $1\dx 227 \dx 227 \dx 3$ & conv  & 426us & 495GF/s & 7.50\\ 
11 & 4 & 96 & $1\dx 227 \dx 227 \dx 3$ & tconv  & 150us & 1.41TF/s & 21.3\\ 
11 & 4 & 96 & $5\dx 224 \dx 224 \dx 3$ & conv  & 1.09ms & 935GF/s & 14.2\\ 
11 & 4 & 96 & $5\dx 224 \dx 224 \dx 3$ & tconv  & 402us & 2.52TF/s & 38.3\\ 
11 & 4 & 96 & $5\dx 227 \dx 227 \dx 3$ & conv  & 1.06ms & 992GF/s & 15.0\\ 
11 & 4 & 96 & $5\dx 227 \dx 227 \dx 3$ & tconv  & 452us & 2.33TF/s & 35.4\\ 
11 & 4 & 96 & $20\dx 224 \dx 224 \dx 3$ & conv  & 3.63ms & 1.12TF/s & 17.0\\ 
11 & 4 & 96 & $20\dx 224 \dx 224 \dx 3$ & tconv  & 1.41ms & 2.88TF/s & 43.6\\ 
11 & 4 & 96 & $20\dx 227 \dx 227 \dx 3$ & conv  & 3.79ms & 1.11TF/s & 16.9\\ 
11 & 4 & 96 & $20\dx 227 \dx 227 \dx 3$ & tconv  & 1.76ms & 2.39TF/s & 36.2\\ 
1 & 1 & 96 & $1\dx 14 \dx 14 \dx 480$ & conv  & 353us & 51.1GF/s & 775m\\ 
1 & 1 & 96 & $1\dx 14 \dx 14 \dx 480$ & k1conv  & 101us & 178GF/s & 2.70\\ 
1 & 1 & 96 & $5\dx 14 \dx 14 \dx 480$ & conv  & 352us & 256GF/s & 3.89\\ 
1 & 1 & 96 & $5\dx 14 \dx 14 \dx 480$ & k1conv  & 101us & 890GF/s & 13.5\\ 
1 & 1 & 96 & $20\dx 14 \dx 14 \dx 480$ & conv  & 514us & 703GF/s & 10.7\\ 
1 & 1 & 96 & $20\dx 14 \dx 14 \dx 480$ & k1conv  & 188us & 1.92TF/s & 29.1\\ 
5 & 1 & 96 & $1\dx 28 \dx 28 \dx 32$ & conv  & 722us & 167GF/s & 2.53\\ 
5 & 1 & 96 & $1\dx 28 \dx 28 \dx 32$ & tconv  & 168us & 717GF/s & 10.9\\ 
5 & 1 & 96 & $5\dx 28 \dx 28 \dx 32$ & conv  & 795us & 758GF/s & 11.5\\ 
5 & 1 & 96 & $5\dx 28 \dx 28 \dx 32$ & tconv  & 267us & 2.25TF/s & 34.1\\ 
5 & 1 & 96 & $20\dx 28 \dx 28 \dx 32$ & conv  & 1.89ms & 1.27TF/s & 19.3\\ 
5 & 1 & 96 & $20\dx 28 \dx 28 \dx 32$ & tconv  & 913us & 2.64TF/s & 40.0\\ 
1 & 1 & 112 & $1\dx 14 \dx 14 \dx 512$ & conv  & 376us & 59.8GF/s & 906m\\ 
1 & 1 & 112 & $1\dx 14 \dx 14 \dx 512$ & k1conv  & 411us & 54.7GF/s & 830m\\ 
1 & 1 & 112 & $5\dx 14 \dx 14 \dx 512$ & conv  & 376us & 299GF/s & 4.53\\ 
1 & 1 & 112 & $5\dx 14 \dx 14 \dx 512$ & k1conv  & 110us & 1.03TF/s & 15.5\\ 
1 & 1 & 112 & $20\dx 14 \dx 14 \dx 512$ & conv  & 549us & 819GF/s & 12.4\\ 
1 & 1 & 112 & $20\dx 14 \dx 14 \dx 512$ & k1conv  & 197us & 2.29TF/s & 34.6\\ 
1 & 1 & 128 & $1\dx 28 \dx 28 \dx 256$ & conv  & 202us & 255GF/s & 3.86\\ 
1 & 1 & 128 & $1\dx 28 \dx 28 \dx 256$ & k1conv  & 70.7us & 727GF/s & 11.0\\ 
1 & 1 & 128 & $5\dx 28 \dx 28 \dx 256$ & conv  & 315us & 817GF/s & 12.4\\ 
1 & 1 & 128 & $5\dx 28 \dx 28 \dx 256$ & k1conv  & 139us & 1.85TF/s & 28.0\\ 
1 & 1 & 128 & $20\dx 28 \dx 28 \dx 256$ & conv  & 1.10ms & 935GF/s & 14.2\\ 
1 & 1 & 128 & $20\dx 28 \dx 28 \dx 256$ & k1conv  & 422us & 2.44TF/s & 36.9\\ 
1 & 1 & 128 & $1\dx 4 \dx 4 \dx 512$ & conv  & 469us & 4.47GF/s & 67.8m\\ 
1 & 1 & 128 & $1\dx 4 \dx 4 \dx 512$ & conv  & 468us & 4.48GF/s & 67.9m\\ 
1 & 1 & 128 & $1\dx 14 \dx 14 \dx 512$ & conv  & 375us & 68.5GF/s & 1.04\\ 
1 & 1 & 128 & $1\dx 14 \dx 14 \dx 512$ & k1conv  & 108us & 239GF/s & 3.62\\ 
1 & 1 & 128 & $5\dx 4 \dx 4 \dx 512$ & conv  & 417us & 25.2GF/s & 381m\\ 
1 & 1 & 128 & $5\dx 4 \dx 4 \dx 512$ & conv  & 373us & 28.1GF/s & 426m\\ 
1 & 1 & 128 & $5\dx 14 \dx 14 \dx 512$ & conv  & 377us & 341GF/s & 5.16\\ 
1 & 1 & 128 & $5\dx 14 \dx 14 \dx 512$ & k1conv  & 112us & 1.15TF/s & 17.4\\ 
1 & 1 & 128 & $20\dx 4 \dx 4 \dx 512$ & conv  & 373us & 113GF/s & 1.71\\ 
1 & 1 & 128 & $20\dx 4 \dx 4 \dx 512$ & conv  & 375us & 112GF/s & 1.70\\ 
1 & 1 & 128 & $20\dx 14 \dx 14 \dx 512$ & conv  & 559us & 919GF/s & 13.9\\ 
1 & 1 & 128 & $20\dx 14 \dx 14 \dx 512$ & k1conv  & 205us & 2.51TF/s & 38.0\\ 
1 & 1 & 128 & $1\dx 4 \dx 4 \dx 528$ & conv  & 484us & 4.47GF/s & 67.7m\\ 
1 & 1 & 128 & $1\dx 4 \dx 4 \dx 528$ & conv  & 484us & 4.47GF/s & 67.7m\\ 
1 & 1 & 128 & $1\dx 14 \dx 14 \dx 528$ & conv  & 385us & 68.8GF/s & 1.04\\ 
1 & 1 & 128 & $1\dx 14 \dx 14 \dx 528$ & k1conv  & 111us & 240GF/s & 3.63\\ 
1 & 1 & 128 & $5\dx 4 \dx 4 \dx 528$ & conv  & 379us & 28.5GF/s & 432m\\ 
1 & 1 & 128 & $5\dx 4 \dx 4 \dx 528$ & conv  & 380us & 28.5GF/s & 431m\\ 
1 & 1 & 128 & $5\dx 14 \dx 14 \dx 528$ & conv  & 389us & 340GF/s & 5.16\\ 
1 & 1 & 128 & $5\dx 14 \dx 14 \dx 528$ & k1conv  & 125us & 1.06TF/s & 16.1\\ 
1 & 1 & 128 & $20\dx 4 \dx 4 \dx 528$ & conv  & 379us & 114GF/s & 1.73\\ 
1 & 1 & 128 & $20\dx 4 \dx 4 \dx 528$ & conv  & 380us & 114GF/s & 1.72\\ 
1 & 1 & 128 & $20\dx 14 \dx 14 \dx 528$ & conv  & 573us & 925GF/s & 14.0\\ 
1 & 1 & 128 & $20\dx 14 \dx 14 \dx 528$ & k1conv  & 208us & 2.55TF/s & 38.6\\ 
5 & 1 & 128 & $1\dx 7 \dx 7 \dx 32$ & conv  & 705us & 14.2GF/s & 216m\\ 
5 & 1 & 128 & $1\dx 7 \dx 7 \dx 32$ & tconv  & 159us & 62.9GF/s & 953m\\ 
5 & 1 & 128 & $1\dx 14 \dx 14 \dx 32$ & conv  & 706us & 56.8GF/s & 861m\\ 
5 & 1 & 128 & $1\dx 14 \dx 14 \dx 32$ & tconv  & 175us & 229GF/s & 3.47\\ 
5 & 1 & 128 & $5\dx 7 \dx 7 \dx 32$ & conv  & 780us & 64.4GF/s & 975m\\ 
5 & 1 & 128 & $5\dx 7 \dx 7 \dx 32$ & tconv  & 159us & 316GF/s & 4.79\\ 
5 & 1 & 128 & $5\dx 14 \dx 14 \dx 32$ & conv  & 709us & 283GF/s & 4.29\\ 
5 & 1 & 128 & $5\dx 14 \dx 14 \dx 32$ & tconv  & 177us & 1.13TF/s & 17.1\\ 
5 & 1 & 128 & $20\dx 7 \dx 7 \dx 32$ & conv  & 709us & 283GF/s & 4.29\\ 
5 & 1 & 128 & $20\dx 7 \dx 7 \dx 32$ & tconv  & 162us & 1.24TF/s & 18.7\\ 
5 & 1 & 128 & $20\dx 14 \dx 14 \dx 32$ & conv  & 789us & 1.02TF/s & 15.4\\ 
5 & 1 & 128 & $20\dx 14 \dx 14 \dx 32$ & tconv  & 294us & 2.73TF/s & 41.4\\ 
1 & 1 & 128 & $1\dx 7 \dx 7 \dx 832$ & conv  & 623us & 16.8GF/s & 254m\\ 
1 & 1 & 128 & $1\dx 7 \dx 7 \dx 832$ & k1conv  & 153us & 68.4GF/s & 1.04\\ 
1 & 1 & 128 & $5\dx 7 \dx 7 \dx 832$ & conv  & 588us & 88.7GF/s & 1.34\\ 
1 & 1 & 128 & $5\dx 7 \dx 7 \dx 832$ & k1conv  & 158us & 331GF/s & 5.02\\ 
1 & 1 & 128 & $20\dx 7 \dx 7 \dx 832$ & conv  & 733us & 285GF/s & 4.31\\ 
1 & 1 & 128 & $20\dx 7 \dx 7 \dx 832$ & k1conv  & 187us & 1.12TF/s & 16.9\\ 
3 & 1 & 128 & $1\dx 28 \dx 28 \dx 96$ & conv  & 788us & 220GF/s & 3.33\\ 
3 & 1 & 128 & $1\dx 28 \dx 28 \dx 96$ & tconv  & 254us & 683GF/s & 10.3\\ 
3 & 1 & 128 & $5\dx 28 \dx 28 \dx 96$ & conv  & 937us & 925GF/s & 14.0\\ 
3 & 1 & 128 & $5\dx 28 \dx 28 \dx 96$ & tconv  & 375us & 2.31TF/s & 35.0\\ 
3 & 1 & 128 & $20\dx 28 \dx 28 \dx 96$ & conv  & 3.07ms & 1.13TF/s & 17.1\\ 
3 & 1 & 128 & $20\dx 28 \dx 28 \dx 96$ & tconv  & 1.23ms & 2.82TF/s & 42.8\\ 
5 & 1 & 128 & $1\dx 7 \dx 7 \dx 48$ & conv  & 1.05ms & 14.4GF/s & 218m\\ 
5 & 1 & 128 & $1\dx 7 \dx 7 \dx 48$ & tconv  & 227us & 66.2GF/s & 1.00\\ 
5 & 1 & 128 & $5\dx 7 \dx 7 \dx 48$ & conv  & 1.05ms & 72.0GF/s & 1.09\\ 
5 & 1 & 128 & $5\dx 7 \dx 7 \dx 48$ & tconv  & 225us & 334GF/s & 5.06\\ 
5 & 1 & 128 & $20\dx 7 \dx 7 \dx 48$ & conv  & 1.05ms & 287GF/s & 4.34\\ 
5 & 1 & 128 & $20\dx 7 \dx 7 \dx 48$ & tconv  & 229us & 1.31TF/s & 19.9\\ 
1 & 1 & 144 & $1\dx 14 \dx 14 \dx 512$ & conv  & 374us & 77.3GF/s & 1.17\\ 
1 & 1 & 144 & $1\dx 14 \dx 14 \dx 512$ & k1conv  & 108us & 269GF/s & 4.07\\ 
1 & 1 & 144 & $5\dx 14 \dx 14 \dx 512$ & conv  & 415us & 349GF/s & 5.28\\ 
1 & 1 & 144 & $5\dx 14 \dx 14 \dx 512$ & k1conv  & 152us & 953GF/s & 14.4\\ 
1 & 1 & 144 & $20\dx 14 \dx 14 \dx 512$ & conv  & 1.03ms & 563GF/s & 8.53\\ 
1 & 1 & 144 & $20\dx 14 \dx 14 \dx 512$ & k1conv  & 326us & 1.77TF/s & 26.8\\ 
1 & 1 & 160 & $1\dx 14 \dx 14 \dx 512$ & conv  & 374us & 85.8GF/s & 1.30\\ 
1 & 1 & 160 & $1\dx 14 \dx 14 \dx 512$ & k1conv  & 108us & 299GF/s & 4.52\\ 
1 & 1 & 160 & $5\dx 14 \dx 14 \dx 512$ & conv  & 424us & 379GF/s & 5.74\\ 
1 & 1 & 160 & $5\dx 14 \dx 14 \dx 512$ & k1conv  & 151us & 1.06TF/s & 16.1\\ 
1 & 1 & 160 & $20\dx 14 \dx 14 \dx 512$ & conv  & 1.04ms & 620GF/s & 9.39\\ 
1 & 1 & 160 & $20\dx 14 \dx 14 \dx 512$ & k1conv  & 336us & 1.91TF/s & 28.9\\ 
1 & 1 & 160 & $1\dx 14 \dx 14 \dx 528$ & conv  & 382us & 86.7GF/s & 1.31\\ 
1 & 1 & 160 & $1\dx 14 \dx 14 \dx 528$ & k1conv  & 106us & 311GF/s & 4.71\\ 
1 & 1 & 160 & $5\dx 14 \dx 14 \dx 528$ & conv  & 454us & 365GF/s & 5.53\\ 
1 & 1 & 160 & $5\dx 14 \dx 14 \dx 528$ & k1conv  & 152us & 1.09TF/s & 16.5\\ 
1 & 1 & 160 & $20\dx 14 \dx 14 \dx 528$ & conv  & 1.06ms & 627GF/s & 9.50\\ 
1 & 1 & 160 & $20\dx 14 \dx 14 \dx 528$ & k1conv  & 335us & 1.98TF/s & 29.9\\ 
1 & 1 & 160 & $1\dx 7 \dx 7 \dx 832$ & conv  & 589us & 22.2GF/s & 336m\\ 
1 & 1 & 160 & $1\dx 7 \dx 7 \dx 832$ & k1conv  & 148us & 87.9GF/s & 1.33\\ 
1 & 1 & 160 & $5\dx 7 \dx 7 \dx 832$ & conv  & 596us & 109GF/s & 1.66\\ 
1 & 1 & 160 & $5\dx 7 \dx 7 \dx 832$ & k1conv  & 151us & 433GF/s & 6.57\\ 
1 & 1 & 160 & $20\dx 7 \dx 7 \dx 832$ & conv  & 763us & 342GF/s & 5.18\\ 
1 & 1 & 160 & $20\dx 7 \dx 7 \dx 832$ & k1conv  & 211us & 1.23TF/s & 18.7\\ 
1 & 1 & 192 & $1\dx 14 \dx 14 \dx 480$ & conv  & 352us & 103GF/s & 1.55\\ 
1 & 1 & 192 & $1\dx 14 \dx 14 \dx 480$ & k1conv  & 98.4us & 367GF/s & 5.56\\ 
1 & 1 & 192 & $5\dx 14 \dx 14 \dx 480$ & conv  & 402us & 449GF/s & 6.81\\ 
1 & 1 & 192 & $5\dx 14 \dx 14 \dx 480$ & k1conv  & 141us & 1.28TF/s & 19.4\\ 
1 & 1 & 192 & $20\dx 14 \dx 14 \dx 480$ & conv  & 1.01ms & 714GF/s & 10.8\\ 
1 & 1 & 192 & $20\dx 14 \dx 14 \dx 480$ & k1conv  & 322us & 2.25TF/s & 34.0\\ 
3 & 1 & 192 & $1\dx 56 \dx 56 \dx 64$ & conv  & 715us & 970GF/s & 14.7\\ 
3 & 1 & 192 & $1\dx 56 \dx 56 \dx 64$ & tconv  & 467us & 1.49TF/s & 22.5\\ 
3 & 1 & 192 & $5\dx 56 \dx 56 \dx 64$ & conv  & 3.27ms & 1.06TF/s & 16.1\\ 
3 & 1 & 192 & $5\dx 56 \dx 56 \dx 64$ & tconv  & 1.59ms & 2.18TF/s & 33.1\\ 
3 & 1 & 192 & $20\dx 56 \dx 56 \dx 64$ & conv  & 11.3ms & 1.23TF/s & 18.7\\ 
3 & 1 & 192 & $20\dx 56 \dx 56 \dx 64$ & tconv  & 5.75ms & 2.41TF/s & 36.6\\ 
1 & 1 & 192 & $1\dx 7 \dx 7 \dx 832$ & conv  & 588us & 26.6GF/s & 404m\\ 
1 & 1 & 192 & $1\dx 7 \dx 7 \dx 832$ & k1conv  & 149us & 105GF/s & 1.60\\ 
1 & 1 & 192 & $5\dx 7 \dx 7 \dx 832$ & conv  & 594us & 132GF/s & 2.00\\ 
1 & 1 & 192 & $5\dx 7 \dx 7 \dx 832$ & k1conv  & 151us & 518GF/s & 7.84\\ 
1 & 1 & 192 & $20\dx 7 \dx 7 \dx 832$ & conv  & 760us & 412GF/s & 6.24\\ 
1 & 1 & 192 & $20\dx 7 \dx 7 \dx 832$ & k1conv  & 207us & 1.52TF/s & 23.0\\ 
3 & 1 & 192 & $1\dx 28 \dx 28 \dx 128$ & conv  & 1.05ms & 332GF/s & 5.03\\ 
3 & 1 & 192 & $1\dx 28 \dx 28 \dx 128$ & tconv  & 367us & 944GF/s & 14.3\\ 
3 & 1 & 192 & $5\dx 28 \dx 28 \dx 128$ & conv  & 2.37ms & 731GF/s & 11.1\\ 
3 & 1 & 192 & $5\dx 28 \dx 28 \dx 128$ & tconv  & 999us & 1.74TF/s & 26.3\\ 
3 & 1 & 192 & $20\dx 28 \dx 28 \dx 128$ & conv  & 6.37ms & 1.09TF/s & 16.5\\ 
3 & 1 & 192 & $20\dx 28 \dx 28 \dx 128$ & tconv  & 3.04ms & 2.28TF/s & 34.6\\ 
3 & 1 & 208 & $1\dx 14 \dx 14 \dx 96$ & conv  & 783us & 89.9GF/s & 1.36\\ 
3 & 1 & 208 & $1\dx 14 \dx 14 \dx 96$ & tconv  & 254us & 277GF/s & 4.20\\ 
3 & 1 & 208 & $5\dx 14 \dx 14 \dx 96$ & conv  & 830us & 424GF/s & 6.43\\ 
3 & 1 & 208 & $5\dx 14 \dx 14 \dx 96$ & tconv  & 301us & 1.17TF/s & 17.7\\ 
3 & 1 & 208 & $20\dx 14 \dx 14 \dx 96$ & conv  & 1.92ms & 733GF/s & 11.1\\ 
3 & 1 & 208 & $20\dx 14 \dx 14 \dx 96$ & tconv  & 738us & 1.91TF/s & 28.9\\ 
3 & 1 & 224 & $1\dx 14 \dx 14 \dx 112$ & conv  & 909us & 97.3GF/s & 1.47\\ 
3 & 1 & 224 & $1\dx 14 \dx 14 \dx 112$ & tconv  & 291us & 304GF/s & 4.61\\ 
3 & 1 & 224 & $5\dx 14 \dx 14 \dx 112$ & conv  & 951us & 465GF/s & 7.05\\ 
3 & 1 & 224 & $5\dx 14 \dx 14 \dx 112$ & tconv  & 356us & 1.24TF/s & 18.8\\ 
3 & 1 & 224 & $20\dx 14 \dx 14 \dx 112$ & conv  & 2.21ms & 802GF/s & 12.1\\ 
3 & 1 & 224 & $20\dx 14 \dx 14 \dx 112$ & tconv  & 844us & 2.10TF/s & 31.8\\ 
1 & 1 & 256 & $1\dx 27 \dx 27 \dx 256$ & conv  & 205us & 467GF/s & 7.07\\ 
1 & 1 & 256 & $1\dx 27 \dx 27 \dx 256$ & k1conv  & 74.8us & 1.28TF/s & 19.4\\ 
1 & 1 & 256 & $5\dx 27 \dx 27 \dx 256$ & conv  & 436us & 1.10TF/s & 16.6\\ 
1 & 1 & 256 & $5\dx 27 \dx 27 \dx 256$ & k1conv  & 206us & 2.32TF/s & 35.2\\ 
1 & 1 & 256 & $20\dx 27 \dx 27 \dx 256$ & conv  & 1.61ms & 1.19TF/s & 18.0\\ 
1 & 1 & 256 & $20\dx 27 \dx 27 \dx 256$ & k1conv  & 654us & 2.92TF/s & 44.3\\ 
1 & 1 & 256 & $1\dx 14 \dx 14 \dx 528$ & conv  & 355us & 149GF/s & 2.26\\ 
1 & 1 & 256 & $1\dx 14 \dx 14 \dx 528$ & k1conv  & 99.3us & 533GF/s & 8.08\\ 
1 & 1 & 256 & $5\dx 14 \dx 14 \dx 528$ & conv  & 453us & 584GF/s & 8.85\\ 
1 & 1 & 256 & $5\dx 14 \dx 14 \dx 528$ & k1conv  & 142us & 1.86TF/s & 28.2\\ 
1 & 1 & 256 & $20\dx 14 \dx 14 \dx 528$ & conv  & 1.14ms & 932GF/s & 14.1\\ 
1 & 1 & 256 & $20\dx 14 \dx 14 \dx 528$ & k1conv  & 354us & 2.99TF/s & 45.3\\ 
1 & 1 & 256 & $1\dx 7 \dx 7 \dx 832$ & conv  & 542us & 38.5GF/s & 584m\\ 
1 & 1 & 256 & $1\dx 7 \dx 7 \dx 832$ & k1conv  & 138us & 151GF/s & 2.29\\ 
1 & 1 & 256 & $5\dx 7 \dx 7 \dx 832$ & conv  & 550us & 190GF/s & 2.88\\ 
1 & 1 & 256 & $5\dx 7 \dx 7 \dx 832$ & k1conv  & 140us & 744GF/s & 11.3\\ 
1 & 1 & 256 & $20\dx 7 \dx 7 \dx 832$ & conv  & 732us & 570GF/s & 8.64\\ 
1 & 1 & 256 & $20\dx 7 \dx 7 \dx 832$ & k1conv  & 197us & 2.12TF/s & 32.2\\ 
3 & 1 & 256 & $1\dx 14 \dx 14 \dx 128$ & conv  & 957us & 121GF/s & 1.83\\ 
3 & 1 & 256 & $1\dx 14 \dx 14 \dx 128$ & tconv  & 304us & 380GF/s & 5.75\\ 
3 & 1 & 256 & $5\dx 14 \dx 14 \dx 128$ & conv  & 982us & 589GF/s & 8.92\\ 
3 & 1 & 256 & $5\dx 14 \dx 14 \dx 128$ & tconv  & 376us & 1.54TF/s & 23.3\\ 
3 & 1 & 256 & $20\dx 14 \dx 14 \dx 128$ & conv  & 2.41ms & 961GF/s & 14.6\\ 
3 & 1 & 256 & $20\dx 14 \dx 14 \dx 128$ & tconv  & 906us & 2.55TF/s & 38.6\\ 
5 & 1 & 256 & $1\dx 27 \dx 27 \dx 96$ & conv  & 2.00ms & 448GF/s & 6.79\\ 
5 & 1 & 256 & $1\dx 27 \dx 27 \dx 96$ & tconv  & 534us & 1.68TF/s & 25.4\\ 
5 & 1 & 256 & $5\dx 27 \dx 27 \dx 96$ & conv  & 2.48ms & 1.81TF/s & 27.4\\ 
5 & 1 & 256 & $5\dx 27 \dx 27 \dx 96$ & tconv  & 1.53ms & 2.93TF/s & 44.4\\ 
5 & 1 & 256 & $20\dx 27 \dx 27 \dx 96$ & conv  & 9.81ms & 1.83TF/s & 27.7\\ 
5 & 1 & 256 & $20\dx 27 \dx 27 \dx 96$ & tconv  & 4.62ms & 3.88TF/s & 58.7\\ 
3 & 1 & 256 & $1\dx 13 \dx 13 \dx 384$ & conv  & 3.29ms & 90.9GF/s & 1.38\\ 
3 & 1 & 256 & $1\dx 13 \dx 13 \dx 384$ & tconv  & 1.05ms & 284GF/s & 4.31\\ 
3 & 1 & 256 & $5\dx 13 \dx 13 \dx 384$ & conv  & 3.13ms & 478GF/s & 7.24\\ 
3 & 1 & 256 & $5\dx 13 \dx 13 \dx 384$ & tconv  & 1.13ms & 1.33TF/s & 20.1\\ 
3 & 1 & 256 & $20\dx 13 \dx 13 \dx 384$ & conv  & 3.55ms & 1.68TF/s & 25.5\\ 
3 & 1 & 256 & $20\dx 13 \dx 13 \dx 384$ & tconv  & 2.56ms & 2.33TF/s & 35.4\\ 
3 & 1 & 288 & $1\dx 14 \dx 14 \dx 144$ & conv  & 1.08ms & 135GF/s & 2.04\\ 
3 & 1 & 288 & $1\dx 14 \dx 14 \dx 144$ & tconv  & 343us & 426GF/s & 6.46\\ 
3 & 1 & 288 & $5\dx 14 \dx 14 \dx 144$ & conv  & 1.32ms & 555GF/s & 8.40\\ 
3 & 1 & 288 & $5\dx 14 \dx 14 \dx 144$ & tconv  & 468us & 1.56TF/s & 23.7\\ 
3 & 1 & 288 & $20\dx 14 \dx 14 \dx 144$ & conv  & 2.71ms & 1.08TF/s & 16.3\\ 
3 & 1 & 288 & $20\dx 14 \dx 14 \dx 144$ & tconv  & 1.46ms & 2.01TF/s & 30.4\\ 
3 & 1 & 320 & $1\dx 7 \dx 7 \dx 160$ & conv  & 1.17ms & 38.5GF/s & 584m\\ 
3 & 1 & 320 & $1\dx 7 \dx 7 \dx 160$ & tconv  & 394us & 115GF/s & 1.74\\ 
3 & 1 & 320 & $1\dx 14 \dx 14 \dx 160$ & conv  & 1.20ms & 151GF/s & 2.29\\ 
3 & 1 & 320 & $1\dx 14 \dx 14 \dx 160$ & tconv  & 380us & 475GF/s & 7.20\\ 
3 & 1 & 320 & $5\dx 7 \dx 7 \dx 160$ & conv  & 1.20ms & 188GF/s & 2.86\\ 
3 & 1 & 320 & $5\dx 7 \dx 7 \dx 160$ & tconv  & 369us & 612GF/s & 9.28\\ 
3 & 1 & 320 & $5\dx 14 \dx 14 \dx 160$ & conv  & 1.47ms & 612GF/s & 9.28\\ 
3 & 1 & 320 & $5\dx 14 \dx 14 \dx 160$ & tconv  & 522us & 1.73TF/s & 26.2\\ 
3 & 1 & 320 & $20\dx 7 \dx 7 \dx 160$ & conv  & 1.48ms & 612GF/s & 9.28\\ 
3 & 1 & 320 & $20\dx 7 \dx 7 \dx 160$ & tconv  & 507us & 1.78TF/s & 27.0\\ 
3 & 1 & 320 & $20\dx 14 \dx 14 \dx 160$ & conv  & 3.02ms & 1.19TF/s & 18.1\\ 
3 & 1 & 320 & $20\dx 14 \dx 14 \dx 160$ & tconv  & 1.64ms & 2.21TF/s & 33.5\\ 
1 & 1 & 384 & $1\dx 13 \dx 13 \dx 384$ & conv  & 265us & 188GF/s & 2.85\\ 
1 & 1 & 384 & $1\dx 13 \dx 13 \dx 384$ & k1conv  & 80.3us & 621GF/s & 9.41\\ 
1 & 1 & 384 & $5\dx 13 \dx 13 \dx 384$ & conv  & 308us & 808GF/s & 12.2\\ 
1 & 1 & 384 & $5\dx 13 \dx 13 \dx 384$ & k1conv  & 116us & 2.15TF/s & 32.6\\ 
1 & 1 & 384 & $20\dx 13 \dx 13 \dx 384$ & conv  & 943us & 1.06TF/s & 16.0\\ 
1 & 1 & 384 & $20\dx 13 \dx 13 \dx 384$ & k1conv  & 318us & 3.13TF/s & 47.4\\ 
1 & 1 & 384 & $1\dx 7 \dx 7 \dx 832$ & conv  & 545us & 57.5GF/s & 871m\\ 
1 & 1 & 384 & $1\dx 7 \dx 7 \dx 832$ & k1conv  & 132us & 237GF/s & 3.59\\ 
1 & 1 & 384 & $5\dx 7 \dx 7 \dx 832$ & conv  & 544us & 288GF/s & 4.36\\ 
1 & 1 & 384 & $5\dx 7 \dx 7 \dx 832$ & k1conv  & 143us & 1.09TF/s & 16.6\\ 
1 & 1 & 384 & $20\dx 7 \dx 7 \dx 832$ & conv  & 762us & 822GF/s & 12.4\\ 
1 & 1 & 384 & $20\dx 7 \dx 7 \dx 832$ & k1conv  & 206us & 3.04TF/s & 46.1\\ 
3 & 1 & 384 & $1\dx 7 \dx 7 \dx 192$ & conv  & 1.41ms & 46.2GF/s & 700m\\ 
3 & 1 & 384 & $1\dx 7 \dx 7 \dx 192$ & tconv  & 434us & 150GF/s & 2.27\\ 
3 & 1 & 384 & $5\dx 7 \dx 7 \dx 192$ & conv  & 1.53ms & 212GF/s & 3.21\\ 
3 & 1 & 384 & $5\dx 7 \dx 7 \dx 192$ & tconv  & 535us & 607GF/s & 9.20\\ 
3 & 1 & 384 & $20\dx 7 \dx 7 \dx 192$ & conv  & 1.75ms & 741GF/s & 11.2\\ 
3 & 1 & 384 & $20\dx 7 \dx 7 \dx 192$ & tconv  & 601us & 2.16TF/s & 32.8\\ 
3 & 1 & 384 & $1\dx 13 \dx 13 \dx 256$ & conv  & 2.21ms & 136GF/s & 2.05\\ 
3 & 1 & 384 & $1\dx 13 \dx 13 \dx 256$ & tconv  & 715us & 418GF/s & 6.34\\ 
3 & 1 & 384 & $5\dx 13 \dx 13 \dx 256$ & conv  & 2.09ms & 715GF/s & 10.8\\ 
3 & 1 & 384 & $5\dx 13 \dx 13 \dx 256$ & tconv  & 789us & 1.89TF/s & 28.7\\ 
3 & 1 & 384 & $20\dx 13 \dx 13 \dx 256$ & conv  & 4.79ms & 1.25TF/s & 18.9\\ 
3 & 1 & 384 & $20\dx 13 \dx 13 \dx 256$ & tconv  & 2.53ms & 2.36TF/s & 35.8\\ 
3 & 1 & 384 & $1\dx 13 \dx 13 \dx 384$ & conv  & 3.30ms & 136GF/s & 2.06\\ 
3 & 1 & 384 & $1\dx 13 \dx 13 \dx 384$ & tconv  & 1.06ms & 422GF/s & 6.39\\ 
3 & 1 & 384 & $5\dx 13 \dx 13 \dx 384$ & conv  & 3.13ms & 717GF/s & 10.9\\ 
3 & 1 & 384 & $5\dx 13 \dx 13 \dx 384$ & tconv  & 1.17ms & 1.92TF/s & 29.1\\ 
3 & 1 & 384 & $20\dx 13 \dx 13 \dx 384$ & conv  & 7.07ms & 1.27TF/s & 19.2\\ 
3 & 1 & 384 & $20\dx 13 \dx 13 \dx 384$ & tconv  & 3.72ms & 2.41TF/s & 36.5\\ 
1 & 1 & 1000 & $1\dx 1 \dx 1 \dx 1024$ & conv  & 679us & 3.02GF/s & 45.7m\\ 
1 & 1 & 1000 & $1\dx 1 \dx 1 \dx 1024$ & conv  & 680us & 3.01GF/s & 45.6m\\ 
1 & 1 & 1000 & $1\dx 6 \dx 6 \dx 1024$ & conv  & 819us & 90.0GF/s & 1.36\\ 
1 & 1 & 1000 & $1\dx 6 \dx 6 \dx 1024$ & k1conv  & 231us & 319GF/s & 4.84\\ 
1 & 1 & 1000 & $5\dx 1 \dx 1 \dx 1024$ & conv  & 1.09ms & 9.38GF/s & 142m\\ 
1 & 1 & 1000 & $5\dx 1 \dx 1 \dx 1024$ & conv  & 1.06ms & 9.68GF/s & 147m\\ 
1 & 1 & 1000 & $5\dx 6 \dx 6 \dx 1024$ & conv  & 816us & 452GF/s & 6.84\\ 
1 & 1 & 1000 & $5\dx 6 \dx 6 \dx 1024$ & k1conv  & 202us & 1.83TF/s & 27.7\\ 
1 & 1 & 1000 & $20\dx 1 \dx 1 \dx 1024$ & conv  & 811us & 50.5GF/s & 766m\\ 
1 & 1 & 1000 & $20\dx 1 \dx 1 \dx 1024$ & conv  & 811us & 50.5GF/s & 765m\\ 
1 & 1 & 1000 & $20\dx 6 \dx 6 \dx 1024$ & conv  & 1.05ms & 1.41TF/s & 21.3\\ 
1 & 1 & 1000 & $20\dx 6 \dx 6 \dx 1024$ & k1conv  & 378us & 3.90TF/s & 59.2\\ 
1 & 1 & 1000 & $1\dx 1 \dx 1 \dx 4096$ & conv  & 2.75ms & 2.98GF/s & 45.2m\\ 
1 & 1 & 1000 & $1\dx 1 \dx 1 \dx 4096$ & conv  & 2.70ms & 3.03GF/s & 46.0m\\ 
1 & 1 & 1000 & $5\dx 1 \dx 1 \dx 4096$ & conv  & 4.19ms & 9.78GF/s & 148m\\ 
1 & 1 & 1000 & $5\dx 1 \dx 1 \dx 4096$ & conv  & 4.18ms & 9.80GF/s & 148m\\ 
1 & 1 & 1000 & $20\dx 1 \dx 1 \dx 4096$ & conv  & 3.16ms & 51.9GF/s & 786m\\ 
1 & 1 & 1000 & $20\dx 1 \dx 1 \dx 4096$ & conv  & 3.16ms & 51.9GF/s & 786m\\ 
1 & 1 & 1024 & $1\dx 6 \dx 6 \dx 1024$ & conv  & 822us & 91.8GF/s & 1.39\\ 
1 & 1 & 1024 & $1\dx 6 \dx 6 \dx 1024$ & k1conv  & 231us & 327GF/s & 4.95\\ 
1 & 1 & 1024 & $5\dx 6 \dx 6 \dx 1024$ & conv  & 818us & 461GF/s & 6.99\\ 
1 & 1 & 1024 & $5\dx 6 \dx 6 \dx 1024$ & k1conv  & 202us & 1.87TF/s & 28.3\\ 
1 & 1 & 1024 & $20\dx 6 \dx 6 \dx 1024$ & conv  & 1.06ms & 1.43TF/s & 21.7\\ 
1 & 1 & 1024 & $20\dx 6 \dx 6 \dx 1024$ & k1conv  & 376us & 4.02TF/s & 60.9\\ 
4 & 1 & 1024 & $1\dx 4 \dx 4 \dx 128$ & conv  & 1.57ms & 2.66GF/s & 40.4m\\ 
4 & 1 & 1024 & $1\dx 4 \dx 4 \dx 128$ & conv  & 1.53ms & 2.74GF/s & 41.5m\\ 
4 & 1 & 1024 & $5\dx 4 \dx 4 \dx 128$ & conv  & 2.20ms & 9.51GF/s & 144m\\ 
4 & 1 & 1024 & $5\dx 4 \dx 4 \dx 128$ & conv  & 2.21ms & 9.50GF/s & 144m\\ 
4 & 1 & 1024 & $20\dx 4 \dx 4 \dx 128$ & conv  & 1.75ms & 47.9GF/s & 725m\\ 
4 & 1 & 1024 & $20\dx 4 \dx 4 \dx 128$ & conv  & 1.76ms & 47.8GF/s & 724m\\ 
3 & 1 & 1024 & $1\dx 6 \dx 6 \dx 384$ & conv  & 3.31ms & 77.1GF/s & 1.17\\ 
3 & 1 & 1024 & $1\dx 6 \dx 6 \dx 384$ & tconv  & 1.02ms & 251GF/s & 3.80\\ 
3 & 1 & 1024 & $5\dx 6 \dx 6 \dx 384$ & conv  & 3.30ms & 386GF/s & 5.85\\ 
3 & 1 & 1024 & $5\dx 6 \dx 6 \dx 384$ & tconv  & 1.07ms & 1.20TF/s & 18.1\\ 
3 & 1 & 1024 & $20\dx 6 \dx 6 \dx 384$ & conv  & 3.59ms & 1.42TF/s & 21.5\\ 
3 & 1 & 1024 & $20\dx 6 \dx 6 \dx 384$ & tconv  & 1.29ms & 3.94TF/s & 59.7\\ 
1 & 1 & 4096 & $1\dx 1 \dx 1 \dx 4096$ & conv  & 2.87ms & 11.7GF/s & 177m\\ 
1 & 1 & 4096 & $1\dx 1 \dx 1 \dx 4096$ & conv  & 2.87ms & 11.7GF/s & 177m\\ 
1 & 1 & 4096 & $5\dx 1 \dx 1 \dx 4096$ & conv  & 4.32ms & 38.9GF/s & 589m\\ 
1 & 1 & 4096 & $5\dx 1 \dx 1 \dx 4096$ & conv  & 4.21ms & 39.8GF/s & 603m\\ 
1 & 1 & 4096 & $20\dx 1 \dx 1 \dx 4096$ & conv  & 3.18ms & 211GF/s & 3.20\\ 
1 & 1 & 4096 & $20\dx 1 \dx 1 \dx 4096$ & conv  & 3.18ms & 211GF/s & 3.20\\ 
6 & 1 & 4096 & $1\dx 6 \dx 6 \dx 256$ & conv  & 8.34ms & 9.05GF/s & 137m\\ 
6 & 1 & 4096 & $1\dx 6 \dx 6 \dx 256$ & conv  & 8.34ms & 9.06GF/s & 137m\\ 
6 & 1 & 4096 & $5\dx 6 \dx 6 \dx 256$ & conv  & 10.5ms & 36.0GF/s & 546m\\ 
6 & 1 & 4096 & $5\dx 6 \dx 6 \dx 256$ & conv  & 10.7ms & 35.4GF/s & 536m\\ 
6 & 1 & 4096 & $20\dx 6 \dx 6 \dx 256$ & conv  & 7.87ms & 192GF/s & 2.91\\ 
6 & 1 & 4096 & $20\dx 6 \dx 6 \dx 256$ & conv  & 7.85ms & 192GF/s & 2.91\\ 


==> op-eff-tab.tex <==
1 & 1 & 256 & $20\dx 13 \dx 13 \dx 256$ & conv  & 591us & 750GF/s & 11.4\\ 
1 & 1 & 256 & $20\dx 13 \dx 13 \dx 256$ & k1conv  & 256us & 1.73TF/s & 26.2\\ 
3 & 1 & 256 & $20\dx 13 \dx 13 \dx 128$ & conv  & 2.44ms & 1.63TF/s & 24.7\\ 
3 & 1 & 256 & $20\dx 13 \dx 13 \dx 128$ & tconv  & 1.24ms & 3.21TF/s & 48.6\\ 
7 & 2 & 96 & $20\dx 205 \dx 205 \dx 3$ & conv  & 8.23ms & 686GF/s & 10.4\\ 
7 & 2 & 96 & $20\dx 205 \dx 205 \dx 3$ & tconv  & 3.68ms & 1.53TF/s & 23.2\\ 


==> op-info-tab.full.tex <==
1 & 1 & 16 & 1 & $28 \dx 28 \dx 192$ & $28 \dx 28 \dx 16$ & 665KB & 4.82MF & 7.25 & $784 \dx 192 \dx 16$\\ 
1 & 1 & 16 & 5 & $28 \dx 28 \dx 192$ & $28 \dx 28 \dx 16$ & 3.27MB & 24.1MF & 7.36 & $3920 \dx 192 \dx 16$\\ 
1 & 1 & 16 & 20 & $28 \dx 28 \dx 192$ & $28 \dx 28 \dx 16$ & 13.1MB & 96.3MF & 7.38 & $15680 \dx 192 \dx 16$\\ 
1 & 1 & 16 & 1 & $14 \dx 14 \dx 480$ & $14 \dx 14 \dx 16$ & 420KB & 3.01MF & 7.17 & $196 \dx 480 \dx 16$\\ 
1 & 1 & 16 & 5 & $14 \dx 14 \dx 480$ & $14 \dx 14 \dx 16$ & 1.98MB & 15.1MF & 7.62 & $980 \dx 480 \dx 16$\\ 
1 & 1 & 16 & 20 & $14 \dx 14 \dx 480$ & $14 \dx 14 \dx 16$ & 7.81MB & 60.2MF & 7.71 & $3920 \dx 480 \dx 16$\\ 
1 & 1 & 24 & 1 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 24$ & 469KB & 4.82MF & 10.3 & $196 \dx 512 \dx 24$\\ 
1 & 1 & 24 & 5 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 24$ & 2.15MB & 24.1MF & 11.2 & $980 \dx 512 \dx 24$\\ 
1 & 1 & 24 & 20 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 24$ & 8.45MB & 96.3MF & 11.4 & $3920 \dx 512 \dx 24$\\ 
1 & 1 & 32 & 1 & $28 \dx 28 \dx 192$ & $28 \dx 28 \dx 32$ & 727KB & 9.63MF & 13.2 & $784 \dx 192 \dx 32$\\ 
1 & 1 & 32 & 5 & $28 \dx 28 \dx 192$ & $28 \dx 28 \dx 32$ & 3.54MB & 48.2MF & 13.6 & $3920 \dx 192 \dx 32$\\ 
1 & 1 & 32 & 20 & $28 \dx 28 \dx 192$ & $28 \dx 28 \dx 32$ & 14.1MB & 193MF & 13.7 & $15680 \dx 192 \dx 32$\\ 
1 & 1 & 32 & 1 & $28 \dx 28 \dx 256$ & $28 \dx 28 \dx 32$ & 936KB & 12.8MF & 13.7 & $784 \dx 256 \dx 32$\\ 
1 & 1 & 32 & 5 & $28 \dx 28 \dx 256$ & $28 \dx 28 \dx 32$ & 4.55MB & 64.2MF & 14.1 & $3920 \dx 256 \dx 32$\\ 
1 & 1 & 32 & 20 & $28 \dx 28 \dx 256$ & $28 \dx 28 \dx 32$ & 18.1MB & 257MF & 14.2 & $15680 \dx 256 \dx 32$\\ 
5 & 1 & 32 & 1 & $28 \dx 28 \dx 16$ & $28 \dx 28 \dx 32$ & 202KB & 20.1MF & 99.4 & $784 \dx 400 \dx 32$\\ 
5 & 1 & 32 & 5 & $28 \dx 28 \dx 16$ & $28 \dx 28 \dx 32$ & 804KB & 100MF & 125 & $3920 \dx 400 \dx 32$\\ 
5 & 1 & 32 & 20 & $28 \dx 28 \dx 16$ & $28 \dx 28 \dx 32$ & 3.06MB & 401MF & 131 & $15680 \dx 400 \dx 32$\\ 
1 & 1 & 32 & 1 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 32$ & 492KB & 6.42MF & 13.0 & $196 \dx 512 \dx 32$\\ 
1 & 1 & 32 & 5 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 32$ & 2.20MB & 32.1MF & 14.6 & $980 \dx 512 \dx 32$\\ 
1 & 1 & 32 & 20 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 32$ & 8.60MB & 128MF & 14.9 & $3920 \dx 512 \dx 32$\\ 
1 & 1 & 32 & 1 & $14 \dx 14 \dx 528$ & $14 \dx 14 \dx 32$ & 507KB & 6.62MF & 13.1 & $196 \dx 528 \dx 32$\\ 
1 & 1 & 32 & 5 & $14 \dx 14 \dx 528$ & $14 \dx 14 \dx 32$ & 2.26MB & 33.1MF & 14.6 & $980 \dx 528 \dx 32$\\ 
1 & 1 & 32 & 20 & $14 \dx 14 \dx 528$ & $14 \dx 14 \dx 32$ & 8.85MB & 132MF & 15.0 & $3920 \dx 528 \dx 32$\\ 
1 & 1 & 32 & 1 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 32$ & 276KB & 2.61MF & 9.45 & $49 \dx 832 \dx 32$\\ 
1 & 1 & 32 & 5 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 32$ & 953KB & 13.0MF & 13.7 & $245 \dx 832 \dx 32$\\ 
1 & 1 & 32 & 20 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 32$ & 3.49MB & 52.2MF & 14.9 & $980 \dx 832 \dx 32$\\ 
5 & 1 & 48 & 1 & $14 \dx 14 \dx 16$ & $14 \dx 14 \dx 48$ & 127KB & 7.53MF & 59.2 & $196 \dx 400 \dx 48$\\ 
5 & 1 & 48 & 5 & $14 \dx 14 \dx 16$ & $14 \dx 14 \dx 48$ & 328KB & 37.6MF & 115 & $980 \dx 400 \dx 48$\\ 
5 & 1 & 48 & 20 & $14 \dx 14 \dx 16$ & $14 \dx 14 \dx 48$ & 1.08MB & 151MF & 139 & $3920 \dx 400 \dx 48$\\ 
1 & 1 & 48 & 1 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 48$ & 332KB & 3.91MF & 11.8 & $49 \dx 832 \dx 48$\\ 
1 & 1 & 48 & 5 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 48$ & 1.02MB & 19.6MF & 19.1 & $245 \dx 832 \dx 48$\\ 
1 & 1 & 48 & 20 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 48$ & 3.61MB & 78.3MF & 21.7 & $980 \dx 832 \dx 48$\\ 
1 & 1 & 64 & 1 & $56 \dx 56 \dx 64$ & $56 \dx 56 \dx 64$ & 1.62MB & 25.7MF & 15.8 & $3136 \dx 64 \dx 64$\\ 
1 & 1 & 64 & 5 & $56 \dx 56 \dx 64$ & $56 \dx 56 \dx 64$ & 8.04MB & 128MF & 16.0 & $15680 \dx 64 \dx 64$\\ 
1 & 1 & 64 & 20 & $56 \dx 56 \dx 64$ & $56 \dx 56 \dx 64$ & 32.1MB & 514MF & 16.0 & $62720 \dx 64 \dx 64$\\ 
7 & 2 & 64 & 1 & $224 \dx 224 \dx 3$ & $112 \dx 112 \dx 64$ & 3.85MB & 236MF & 61.3 & $12544 \dx 147 \dx 64$\\ 
7 & 2 & 64 & 5 & $224 \dx 224 \dx 3$ & $112 \dx 112 \dx 64$ & 19.1MB & 1.18GF & 61.8 & $62720 \dx 147 \dx 64$\\ 
7 & 2 & 64 & 20 & $224 \dx 224 \dx 3$ & $112 \dx 112 \dx 64$ & 76.3MB & 4.72GF & 61.9 & $250880 \dx 147 \dx 64$\\ 
1 & 1 & 64 & 1 & $28 \dx 28 \dx 192$ & $28 \dx 28 \dx 64$ & 852KB & 19.3MF & 22.6 & $784 \dx 192 \dx 64$\\ 
1 & 1 & 64 & 5 & $28 \dx 28 \dx 192$ & $28 \dx 28 \dx 64$ & 4.06MB & 96.3MF & 23.7 & $3920 \dx 192 \dx 64$\\ 
1 & 1 & 64 & 20 & $28 \dx 28 \dx 192$ & $28 \dx 28 \dx 64$ & 16.1MB & 385MF & 23.9 & $15680 \dx 192 \dx 64$\\ 
1 & 1 & 64 & 1 & $28 \dx 28 \dx 256$ & $28 \dx 28 \dx 64$ & 1.07MB & 25.7MF & 24.0 & $784 \dx 256 \dx 64$\\ 
1 & 1 & 64 & 5 & $28 \dx 28 \dx 256$ & $28 \dx 28 \dx 64$ & 5.08MB & 128MF & 25.3 & $3920 \dx 256 \dx 64$\\ 
1 & 1 & 64 & 20 & $28 \dx 28 \dx 256$ & $28 \dx 28 \dx 64$ & 20.1MB & 514MF & 25.5 & $15680 \dx 256 \dx 64$\\ 
1 & 1 & 64 & 1 & $14 \dx 14 \dx 480$ & $14 \dx 14 \dx 64$ & 550KB & 12.0MF & 21.9 & $196 \dx 480 \dx 64$\\ 
1 & 1 & 64 & 5 & $14 \dx 14 \dx 480$ & $14 \dx 14 \dx 64$ & 2.26MB & 60.2MF & 26.7 & $980 \dx 480 \dx 64$\\ 
1 & 1 & 64 & 20 & $14 \dx 14 \dx 480$ & $14 \dx 14 \dx 64$ & 8.65MB & 241MF & 27.8 & $3920 \dx 480 \dx 64$\\ 
1 & 1 & 64 & 1 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 64$ & 583KB & 12.8MF & 22.0 & $196 \dx 512 \dx 64$\\ 
1 & 1 & 64 & 5 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 64$ & 2.39MB & 64.2MF & 26.9 & $980 \dx 512 \dx 64$\\ 
1 & 1 & 64 & 20 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 64$ & 9.16MB & 257MF & 28.0 & $3920 \dx 512 \dx 64$\\ 
5 & 1 & 64 & 1 & $14 \dx 14 \dx 24$ & $14 \dx 14 \dx 64$ & 223KB & 15.1MF & 67.5 & $196 \dx 600 \dx 64$\\ 
5 & 1 & 64 & 5 & $14 \dx 14 \dx 24$ & $14 \dx 14 \dx 64$ & 499KB & 75.3MF & 151 & $980 \dx 600 \dx 64$\\ 
5 & 1 & 64 & 20 & $14 \dx 14 \dx 24$ & $14 \dx 14 \dx 64$ & 1.53MB & 301MF & 196 & $3920 \dx 600 \dx 64$\\ 
5 & 1 & 64 & 1 & $14 \dx 14 \dx 32$ & $14 \dx 14 \dx 64$ & 280KB & 20.1MF & 71.6 & $196 \dx 800 \dx 64$\\ 
5 & 1 & 64 & 5 & $14 \dx 14 \dx 32$ & $14 \dx 14 \dx 64$ & 581KB & 100MF & 173 & $980 \dx 800 \dx 64$\\ 
5 & 1 & 64 & 20 & $14 \dx 14 \dx 32$ & $14 \dx 14 \dx 64$ & 1.71MB & 401MF & 235 & $3920 \dx 800 \dx 64$\\ 
1 & 1 & 96 & 1 & $54 \dx 54 \dx 96$ & $54 \dx 54 \dx 96$ & 2.28MB & 53.7MF & 23.6 & $2916 \dx 96 \dx 96$\\ 
1 & 1 & 96 & 5 & $54 \dx 54 \dx 96$ & $54 \dx 54 \dx 96$ & 11.2MB & 269MF & 23.9 & $14580 \dx 96 \dx 96$\\ 
1 & 1 & 96 & 20 & $54 \dx 54 \dx 96$ & $54 \dx 54 \dx 96$ & 44.8MB & 1.07GF & 24.0 & $58320 \dx 96 \dx 96$\\ 
1 & 1 & 96 & 1 & $28 \dx 28 \dx 192$ & $28 \dx 28 \dx 96$ & 977KB & 28.9MF & 29.6 & $784 \dx 192 \dx 96$\\ 
1 & 1 & 96 & 5 & $28 \dx 28 \dx 192$ & $28 \dx 28 \dx 96$ & 4.59MB & 145MF & 31.5 & $3920 \dx 192 \dx 96$\\ 
1 & 1 & 96 & 20 & $28 \dx 28 \dx 192$ & $28 \dx 28 \dx 96$ & 18.1MB & 578MF & 31.9 & $15680 \dx 192 \dx 96$\\ 
11 & 4 & 96 & 1 & $224 \dx 224 \dx 3$ & $54 \dx 54 \dx 96$ & 1.86MB & 203MF & 109 & $2916 \dx 363 \dx 96$\\ 
11 & 4 & 96 & 1 & $227 \dx 227 \dx 3$ & $55 \dx 55 \dx 96$ & 1.92MB & 211MF & 110 & $3025 \dx 363 \dx 96$\\ 
11 & 4 & 96 & 5 & $224 \dx 224 \dx 3$ & $54 \dx 54 \dx 96$ & 8.75MB & 1.02GF & 116 & $14580 \dx 363 \dx 96$\\ 
11 & 4 & 96 & 5 & $227 \dx 227 \dx 3$ & $55 \dx 55 \dx 96$ & 9.04MB & 1.05GF & 117 & $15125 \dx 363 \dx 96$\\ 
11 & 4 & 96 & 20 & $224 \dx 224 \dx 3$ & $54 \dx 54 \dx 96$ & 34.6MB & 4.06GF & 118 & $58320 \dx 363 \dx 96$\\ 
11 & 4 & 96 & 20 & $227 \dx 227 \dx 3$ & $55 \dx 55 \dx 96$ & 35.7MB & 4.22GF & 118 & $60500 \dx 363 \dx 96$\\ 
1 & 1 & 96 & 1 & $14 \dx 14 \dx 480$ & $14 \dx 14 \dx 96$ & 636KB & 18.1MF & 28.4 & $196 \dx 480 \dx 96$\\ 
1 & 1 & 96 & 5 & $14 \dx 14 \dx 480$ & $14 \dx 14 \dx 96$ & 2.44MB & 90.3MF & 37.0 & $980 \dx 480 \dx 96$\\ 
1 & 1 & 96 & 20 & $14 \dx 14 \dx 480$ & $14 \dx 14 \dx 96$ & 9.22MB & 361MF & 39.2 & $3920 \dx 480 \dx 96$\\ 
5 & 1 & 96 & 1 & $28 \dx 28 \dx 32$ & $28 \dx 28 \dx 96$ & 709KB & 120MF & 170 & $784 \dx 800 \dx 96$\\ 
5 & 1 & 96 & 5 & $28 \dx 28 \dx 32$ & $28 \dx 28 \dx 96$ & 2.31MB & 602MF & 260 & $3920 \dx 800 \dx 96$\\ 
5 & 1 & 96 & 20 & $28 \dx 28 \dx 32$ & $28 \dx 28 \dx 96$ & 8.34MB & 2.41GF & 289 & $15680 \dx 800 \dx 96$\\ 
1 & 1 & 112 & 1 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 112$ & 719KB & 22.5MF & 31.3 & $196 \dx 512 \dx 112$\\ 
1 & 1 & 112 & 5 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 112$ & 2.68MB & 112MF & 42.0 & $980 \dx 512 \dx 112$\\ 
1 & 1 & 112 & 20 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 112$ & 10.0MB & 450MF & 44.9 & $3920 \dx 512 \dx 112$\\ 
1 & 1 & 128 & 1 & $28 \dx 28 \dx 256$ & $28 \dx 28 \dx 128$ & 1.34MB & 51.4MF & 38.5 & $784 \dx 256 \dx 128$\\ 
1 & 1 & 128 & 5 & $28 \dx 28 \dx 256$ & $28 \dx 28 \dx 128$ & 6.15MB & 257MF & 41.8 & $3920 \dx 256 \dx 128$\\ 
1 & 1 & 128 & 20 & $28 \dx 28 \dx 256$ & $28 \dx 28 \dx 128$ & 24.2MB & 1.03GF & 42.4 & $15680 \dx 256 \dx 128$\\ 
1 & 1 & 128 & 1 & $4 \dx 4 \dx 512$ & $4 \dx 4 \dx 128$ & 304KB & 2.10MF & 6.91 & $16 \dx 512 \dx 128$\\ 
1 & 1 & 128 & 1 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 128$ & 764KB & 25.7MF & 33.6 & $196 \dx 512 \dx 128$\\ 
1 & 1 & 128 & 5 & $4 \dx 4 \dx 512$ & $4 \dx 4 \dx 128$ & 467KB & 10.5MF & 22.4 & $80 \dx 512 \dx 128$\\ 
1 & 1 & 128 & 5 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 128$ & 2.77MB & 128MF & 46.3 & $980 \dx 512 \dx 128$\\ 
1 & 1 & 128 & 20 & $4 \dx 4 \dx 512$ & $4 \dx 4 \dx 128$ & 1.08MB & 41.9MF & 38.8 & $320 \dx 512 \dx 128$\\ 
1 & 1 & 128 & 20 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 128$ & 10.3MB & 514MF & 49.9 & $3920 \dx 512 \dx 128$\\ 
1 & 1 & 128 & 1 & $4 \dx 4 \dx 528$ & $4 \dx 4 \dx 128$ & 313KB & 2.16MF & 6.91 & $16 \dx 528 \dx 128$\\ 
1 & 1 & 128 & 1 & $14 \dx 14 \dx 528$ & $14 \dx 14 \dx 128$ & 785KB & 26.5MF & 33.7 & $196 \dx 528 \dx 128$\\ 
1 & 1 & 128 & 5 & $4 \dx 4 \dx 528$ & $4 \dx 4 \dx 128$ & 481KB & 10.8MF & 22.5 & $80 \dx 528 \dx 128$\\ 
1 & 1 & 128 & 5 & $14 \dx 14 \dx 528$ & $14 \dx 14 \dx 128$ & 2.84MB & 132MF & 46.6 & $980 \dx 528 \dx 128$\\ 
1 & 1 & 128 & 20 & $4 \dx 4 \dx 528$ & $4 \dx 4 \dx 128$ & 1.11MB & 43.3MF & 38.9 & $320 \dx 528 \dx 128$\\ 
1 & 1 & 128 & 20 & $14 \dx 14 \dx 528$ & $14 \dx 14 \dx 128$ & 10.6MB & 530MF & 50.2 & $3920 \dx 528 \dx 128$\\ 
5 & 1 & 128 & 1 & $7 \dx 7 \dx 32$ & $7 \dx 7 \dx 128$ & 441KB & 10.0MF & 22.7 & $49 \dx 800 \dx 128$\\ 
5 & 1 & 128 & 1 & $14 \dx 14 \dx 32$ & $14 \dx 14 \dx 128$ & 536KB & 40.1MF & 75.0 & $196 \dx 800 \dx 128$\\ 
5 & 1 & 128 & 5 & $7 \dx 7 \dx 32$ & $7 \dx 7 \dx 128$ & 567KB & 50.2MF & 88.5 & $245 \dx 800 \dx 128$\\ 
5 & 1 & 128 & 5 & $14 \dx 14 \dx 32$ & $14 \dx 14 \dx 128$ & 1.04MB & 201MF & 193 & $980 \dx 800 \dx 128$\\ 
5 & 1 & 128 & 20 & $7 \dx 7 \dx 32$ & $7 \dx 7 \dx 128$ & 1.04MB & 201MF & 193 & $980 \dx 800 \dx 128$\\ 
5 & 1 & 128 & 20 & $14 \dx 14 \dx 32$ & $14 \dx 14 \dx 128$ & 2.92MB & 803MF & 275 & $3920 \dx 800 \dx 128$\\ 
1 & 1 & 128 & 1 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 128$ & 615KB & 10.4MF & 17.0 & $49 \dx 832 \dx 128$\\ 
1 & 1 & 128 & 5 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 128$ & 1.37MB & 52.2MF & 38.2 & $245 \dx 832 \dx 128$\\ 
1 & 1 & 128 & 20 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 128$ & 4.19MB & 209MF & 49.8 & $980 \dx 832 \dx 128$\\ 
3 & 1 & 128 & 1 & $28 \dx 28 \dx 96$ & $28 \dx 28 \dx 128$ & 1.15MB & 173MF & 151 & $784 \dx 864 \dx 128$\\ 
3 & 1 & 128 & 5 & $28 \dx 28 \dx 96$ & $28 \dx 28 \dx 128$ & 3.96MB & 867MF & 219 & $3920 \dx 864 \dx 128$\\ 
3 & 1 & 128 & 20 & $28 \dx 28 \dx 96$ & $28 \dx 28 \dx 128$ & 14.5MB & 3.47GF & 239 & $15680 \dx 864 \dx 128$\\ 
5 & 1 & 128 & 1 & $7 \dx 7 \dx 48$ & $7 \dx 7 \dx 128$ & 649KB & 15.1MF & 23.2 & $49 \dx 1200 \dx 128$\\ 
5 & 1 & 128 & 5 & $7 \dx 7 \dx 48$ & $7 \dx 7 \dx 128$ & 787KB & 75.3MF & 95.6 & $245 \dx 1200 \dx 128$\\ 
5 & 1 & 128 & 20 & $7 \dx 7 \dx 48$ & $7 \dx 7 \dx 128$ & 1.30MB & 301MF & 231 & $980 \dx 1200 \dx 128$\\ 
1 & 1 & 144 & 1 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 144$ & 810KB & 28.9MF & 35.7 & $196 \dx 512 \dx 144$\\ 
1 & 1 & 144 & 5 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 144$ & 2.87MB & 145MF & 50.4 & $980 \dx 512 \dx 144$\\ 
1 & 1 & 144 & 20 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 144$ & 10.6MB & 578MF & 54.6 & $3920 \dx 512 \dx 144$\\ 
1 & 1 & 160 & 1 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 160$ & 855KB & 32.1MF & 37.6 & $196 \dx 512 \dx 160$\\ 
1 & 1 & 160 & 5 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 160$ & 2.96MB & 161MF & 54.2 & $980 \dx 512 \dx 160$\\ 
1 & 1 & 160 & 20 & $14 \dx 14 \dx 512$ & $14 \dx 14 \dx 160$ & 10.9MB & 642MF & 59.1 & $3920 \dx 512 \dx 160$\\ 
1 & 1 & 160 & 1 & $14 \dx 14 \dx 528$ & $14 \dx 14 \dx 160$ & 878KB & 33.1MF & 37.7 & $196 \dx 528 \dx 160$\\ 
1 & 1 & 160 & 5 & $14 \dx 14 \dx 528$ & $14 \dx 14 \dx 160$ & 3.04MB & 166MF & 54.5 & $980 \dx 528 \dx 160$\\ 
1 & 1 & 160 & 20 & $14 \dx 14 \dx 528$ & $14 \dx 14 \dx 160$ & 11.1MB & 662MF & 59.5 & $3920 \dx 528 \dx 160$\\ 
1 & 1 & 160 & 1 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 160$ & 728KB & 13.0MF & 17.9 & $49 \dx 832 \dx 160$\\ 
1 & 1 & 160 & 5 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 160$ & 1.51MB & 65.2MF & 43.3 & $245 \dx 832 \dx 160$\\ 
1 & 1 & 160 & 20 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 160$ & 4.42MB & 261MF & 59.0 & $980 \dx 832 \dx 160$\\ 
1 & 1 & 192 & 1 & $14 \dx 14 \dx 480$ & $14 \dx 14 \dx 192$ & 896KB & 36.1MF & 40.3 & $196 \dx 480 \dx 192$\\ 
1 & 1 & 192 & 5 & $14 \dx 14 \dx 480$ & $14 \dx 14 \dx 192$ & 3.00MB & 181MF & 60.1 & $980 \dx 480 \dx 192$\\ 
1 & 1 & 192 & 20 & $14 \dx 14 \dx 480$ & $14 \dx 14 \dx 192$ & 10.9MB & 723MF & 66.2 & $3920 \dx 480 \dx 192$\\ 
3 & 1 & 192 & 1 & $56 \dx 56 \dx 64$ & $56 \dx 56 \dx 192$ & 3.65MB & 694MF & 190 & $3136 \dx 576 \dx 192$\\ 
3 & 1 & 192 & 5 & $56 \dx 56 \dx 64$ & $56 \dx 56 \dx 192$ & 16.5MB & 3.47GF & 210 & $15680 \dx 576 \dx 192$\\ 
3 & 1 & 192 & 20 & $56 \dx 56 \dx 64$ & $56 \dx 56 \dx 192$ & 64.7MB & 13.9GF & 215 & $62720 \dx 576 \dx 192$\\ 
1 & 1 & 192 & 1 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 192$ & 840KB & 15.7MF & 18.6 & $49 \dx 832 \dx 192$\\ 
1 & 1 & 192 & 5 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 192$ & 1.64MB & 78.3MF & 47.6 & $245 \dx 832 \dx 192$\\ 
1 & 1 & 192 & 20 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 192$ & 4.65MB & 313MF & 67.3 & $980 \dx 832 \dx 192$\\ 
3 & 1 & 192 & 1 & $28 \dx 28 \dx 128$ & $28 \dx 28 \dx 192$ & 1.89MB & 347MF & 184 & $784 \dx 1152 \dx 192$\\ 
3 & 1 & 192 & 5 & $28 \dx 28 \dx 128$ & $28 \dx 28 \dx 192$ & 5.90MB & 1.73GF & 294 & $3920 \dx 1152 \dx 192$\\ 
3 & 1 & 192 & 20 & $28 \dx 28 \dx 128$ & $28 \dx 28 \dx 192$ & 21.0MB & 6.94GF & 331 & $15680 \dx 1152 \dx 192$\\ 
3 & 1 & 208 & 1 & $14 \dx 14 \dx 96$ & $14 \dx 14 \dx 208$ & 958KB & 70.4MF & 73.5 & $196 \dx 864 \dx 208$\\ 
3 & 1 & 208 & 5 & $14 \dx 14 \dx 96$ & $14 \dx 14 \dx 208$ & 1.91MB & 352MF & 184 & $980 \dx 864 \dx 208$\\ 
3 & 1 & 208 & 20 & $14 \dx 14 \dx 96$ & $14 \dx 14 \dx 208$ & 5.49MB & 1.41GF & 257 & $3920 \dx 864 \dx 208$\\ 
3 & 1 & 224 & 1 & $14 \dx 14 \dx 112$ & $14 \dx 14 \dx 224$ & 1.17MB & 88.5MF & 75.8 & $196 \dx 1008 \dx 224$\\ 
3 & 1 & 224 & 5 & $14 \dx 14 \dx 112$ & $14 \dx 14 \dx 224$ & 2.22MB & 443MF & 199 & $980 \dx 1008 \dx 224$\\ 
3 & 1 & 224 & 20 & $14 \dx 14 \dx 112$ & $14 \dx 14 \dx 224$ & 6.17MB & 1.77GF & 287 & $3920 \dx 1008 \dx 224$\\ 
1 & 1 & 256 & 1 & $27 \dx 27 \dx 256$ & $27 \dx 27 \dx 256$ & 1.76MB & 95.6MF & 54.4 & $729 \dx 256 \dx 256$\\ 
1 & 1 & 256 & 5 & $27 \dx 27 \dx 256$ & $27 \dx 27 \dx 256$ & 7.73MB & 478MF & 61.8 & $3645 \dx 256 \dx 256$\\ 
1 & 1 & 256 & 20 & $27 \dx 27 \dx 256$ & $27 \dx 27 \dx 256$ & 30.1MB & 1.91GF & 63.4 & $14580 \dx 256 \dx 256$\\ 
1 & 1 & 256 & 1 & $14 \dx 14 \dx 528$ & $14 \dx 14 \dx 256$ & 1.16MB & 53.0MF & 45.8 & $196 \dx 528 \dx 256$\\ 
1 & 1 & 256 & 5 & $14 \dx 14 \dx 528$ & $14 \dx 14 \dx 256$ & 3.61MB & 265MF & 73.3 & $980 \dx 528 \dx 256$\\ 
1 & 1 & 256 & 20 & $14 \dx 14 \dx 528$ & $14 \dx 14 \dx 256$ & 12.8MB & 1.06GF & 82.6 & $3920 \dx 528 \dx 256$\\ 
1 & 1 & 256 & 1 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 256$ & 1.07MB & 20.9MF & 19.6 & $49 \dx 832 \dx 256$\\ 
1 & 1 & 256 & 5 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 256$ & 1.92MB & 104MF & 54.4 & $245 \dx 832 \dx 256$\\ 
1 & 1 & 256 & 20 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 256$ & 5.12MB & 417MF & 81.6 & $980 \dx 832 \dx 256$\\ 
3 & 1 & 256 & 1 & $14 \dx 14 \dx 128$ & $14 \dx 14 \dx 256$ & 1.48MB & 116MF & 78.0 & $196 \dx 1152 \dx 256$\\ 
3 & 1 & 256 & 5 & $14 \dx 14 \dx 128$ & $14 \dx 14 \dx 256$ & 2.69MB & 578MF & 215 & $980 \dx 1152 \dx 256$\\ 
3 & 1 & 256 & 20 & $14 \dx 14 \dx 128$ & $14 \dx 14 \dx 256$ & 7.20MB & 2.31GF & 321 & $3920 \dx 1152 \dx 256$\\ 
5 & 1 & 256 & 1 & $27 \dx 27 \dx 96$ & $27 \dx 27 \dx 256$ & 3.49MB & 896MF & 257 & $729 \dx 2400 \dx 256$\\ 
5 & 1 & 256 & 5 & $27 \dx 27 \dx 96$ & $27 \dx 27 \dx 256$ & 7.59MB & 4.48GF & 590 & $3645 \dx 2400 \dx 256$\\ 
5 & 1 & 256 & 20 & $27 \dx 27 \dx 96$ & $27 \dx 27 \dx 256$ & 23.0MB & 17.9GF & 779 & $14580 \dx 2400 \dx 256$\\ 
3 & 1 & 256 & 1 & $13 \dx 13 \dx 384$ & $13 \dx 13 \dx 256$ & 3.97MB & 299MF & 75.3 & $169 \dx 3456 \dx 256$\\ 
3 & 1 & 256 & 5 & $13 \dx 13 \dx 384$ & $13 \dx 13 \dx 256$ & 5.70MB & 1.50GF & 262 & $845 \dx 3456 \dx 256$\\ 
3 & 1 & 256 & 20 & $13 \dx 13 \dx 384$ & $13 \dx 13 \dx 256$ & 12.2MB & 5.98GF & 491 & $3380 \dx 3456 \dx 256$\\ 
3 & 1 & 288 & 1 & $14 \dx 14 \dx 144$ & $14 \dx 14 \dx 288$ & 1.83MB & 146MF & 79.8 & $196 \dx 1296 \dx 288$\\ 
3 & 1 & 288 & 5 & $14 \dx 14 \dx 144$ & $14 \dx 14 \dx 288$ & 3.19MB & 732MF & 230 & $980 \dx 1296 \dx 288$\\ 
3 & 1 & 288 & 20 & $14 \dx 14 \dx 144$ & $14 \dx 14 \dx 288$ & 8.27MB & 2.93GF & 354 & $3920 \dx 1296 \dx 288$\\ 
3 & 1 & 320 & 1 & $7 \dx 7 \dx 160$ & $7 \dx 7 \dx 320$ & 1.94MB & 45.2MF & 23.3 & $49 \dx 1440 \dx 320$\\ 
3 & 1 & 320 & 1 & $14 \dx 14 \dx 160$ & $14 \dx 14 \dx 320$ & 2.22MB & 181MF & 81.3 & $196 \dx 1440 \dx 320$\\ 
3 & 1 & 320 & 5 & $7 \dx 7 \dx 160$ & $7 \dx 7 \dx 320$ & 2.31MB & 226MF & 97.5 & $245 \dx 1440 \dx 320$\\ 
3 & 1 & 320 & 5 & $14 \dx 14 \dx 160$ & $14 \dx 14 \dx 320$ & 3.73MB & 903MF & 242 & $980 \dx 1440 \dx 320$\\ 
3 & 1 & 320 & 20 & $7 \dx 7 \dx 160$ & $7 \dx 7 \dx 320$ & 3.73MB & 903MF & 242 & $980 \dx 1440 \dx 320$\\ 
3 & 1 & 320 & 20 & $14 \dx 14 \dx 160$ & $14 \dx 14 \dx 320$ & 9.37MB & 3.61GF & 386 & $3920 \dx 1440 \dx 320$\\ 
1 & 1 & 384 & 1 & $13 \dx 13 \dx 384$ & $13 \dx 13 \dx 384$ & 1.11MB & 49.8MF & 44.9 & $169 \dx 384 \dx 384$\\ 
1 & 1 & 384 & 5 & $13 \dx 13 \dx 384$ & $13 \dx 13 \dx 384$ & 3.19MB & 249MF & 78.2 & $845 \dx 384 \dx 384$\\ 
1 & 1 & 384 & 20 & $13 \dx 13 \dx 384$ & $13 \dx 13 \dx 384$ & 11.0MB & 997MF & 90.8 & $3380 \dx 384 \dx 384$\\ 
1 & 1 & 384 & 1 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 384$ & 1.52MB & 31.3MF & 20.6 & $49 \dx 832 \dx 384$\\ 
1 & 1 & 384 & 5 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 384$ & 2.47MB & 157MF & 63.4 & $245 \dx 832 \dx 384$\\ 
1 & 1 & 384 & 20 & $7 \dx 7 \dx 832$ & $7 \dx 7 \dx 384$ & 6.05MB & 626MF & 104 & $980 \dx 832 \dx 384$\\ 
3 & 1 & 384 & 1 & $7 \dx 7 \dx 192$ & $7 \dx 7 \dx 384$ & 2.77MB & 65.0MF & 23.5 & $49 \dx 1728 \dx 384$\\ 
3 & 1 & 384 & 5 & $7 \dx 7 \dx 192$ & $7 \dx 7 \dx 384$ & 3.22MB & 325MF & 101 & $245 \dx 1728 \dx 384$\\ 
3 & 1 & 384 & 20 & $7 \dx 7 \dx 192$ & $7 \dx 7 \dx 384$ & 4.91MB & 1.30GF & 265 & $980 \dx 1728 \dx 384$\\ 
3 & 1 & 384 & 1 & $13 \dx 13 \dx 256$ & $13 \dx 13 \dx 384$ & 3.97MB & 299MF & 75.3 & $169 \dx 2304 \dx 384$\\ 
3 & 1 & 384 & 5 & $13 \dx 13 \dx 256$ & $13 \dx 13 \dx 384$ & 5.70MB & 1.50GF & 262 & $845 \dx 2304 \dx 384$\\ 
3 & 1 & 384 & 20 & $13 \dx 13 \dx 256$ & $13 \dx 13 \dx 384$ & 12.2MB & 5.98GF & 491 & $3380 \dx 2304 \dx 384$\\ 
3 & 1 & 384 & 1 & $13 \dx 13 \dx 384$ & $13 \dx 13 \dx 384$ & 5.83MB & 449MF & 77.0 & $169 \dx 3456 \dx 384$\\ 
3 & 1 & 384 & 5 & $13 \dx 13 \dx 384$ & $13 \dx 13 \dx 384$ & 7.91MB & 2.24GF & 284 & $845 \dx 3456 \dx 384$\\ 
3 & 1 & 384 & 20 & $13 \dx 13 \dx 384$ & $13 \dx 13 \dx 384$ & 15.7MB & 8.97GF & 572 & $3380 \dx 3456 \dx 384$\\ 
1 & 1 & 1000 & 1 & $1 \dx 1 \dx 1024$ & $1 \dx 1 \dx 1000$ & 4.11MB & 2.05MF & 499m & $1 \dx 1024 \dx 1000$\\ 
1 & 1 & 1000 & 1 & $6 \dx 6 \dx 1024$ & $6 \dx 6 \dx 1000$ & 4.39MB & 73.7MF & 16.8 & $36 \dx 1024 \dx 1000$\\ 
1 & 1 & 1000 & 5 & $1 \dx 1 \dx 1024$ & $1 \dx 1 \dx 1000$ & 4.14MB & 10.2MF & 2.47 & $5 \dx 1024 \dx 1000$\\ 
1 & 1 & 1000 & 5 & $6 \dx 6 \dx 1024$ & $6 \dx 6 \dx 1000$ & 5.56MB & 369MF & 66.3 & $180 \dx 1024 \dx 1000$\\ 
1 & 1 & 1000 & 20 & $1 \dx 1 \dx 1024$ & $1 \dx 1 \dx 1000$ & 4.26MB & 41.0MF & 9.61 & $20 \dx 1024 \dx 1000$\\ 
1 & 1 & 1000 & 20 & $6 \dx 6 \dx 1024$ & $6 \dx 6 \dx 1000$ & 9.93MB & 1.47GF & 149 & $720 \dx 1024 \dx 1000$\\ 
1 & 1 & 1000 & 1 & $1 \dx 1 \dx 4096$ & $1 \dx 1 \dx 1000$ & 16.4MB & 8.19MF & 499m & $1 \dx 4096 \dx 1000$\\ 
1 & 1 & 1000 & 5 & $1 \dx 1 \dx 4096$ & $1 \dx 1 \dx 1000$ & 16.5MB & 41.0MF & 2.48 & $5 \dx 4096 \dx 1000$\\ 
1 & 1 & 1000 & 20 & $1 \dx 1 \dx 4096$ & $1 \dx 1 \dx 1000$ & 16.8MB & 164MF & 9.75 & $20 \dx 4096 \dx 1000$\\ 
1 & 1 & 1024 & 1 & $6 \dx 6 \dx 1024$ & $6 \dx 6 \dx 1024$ & 4.49MB & 75.5MF & 16.8 & $36 \dx 1024 \dx 1024$\\ 
1 & 1 & 1024 & 5 & $6 \dx 6 \dx 1024$ & $6 \dx 6 \dx 1024$ & 5.67MB & 377MF & 66.5 & $180 \dx 1024 \dx 1024$\\ 
1 & 1 & 1024 & 20 & $6 \dx 6 \dx 1024$ & $6 \dx 6 \dx 1024$ & 10.1MB & 1.51GF & 150 & $720 \dx 1024 \dx 1024$\\ 
4 & 1 & 1024 & 1 & $4 \dx 4 \dx 128$ & $1 \dx 1 \dx 1024$ & 8.40MB & 4.19MF & 499m & $1 \dx 2048 \dx 1024$\\ 
4 & 1 & 1024 & 5 & $4 \dx 4 \dx 128$ & $1 \dx 1 \dx 1024$ & 8.45MB & 21.0MF & 2.48 & $5 \dx 2048 \dx 1024$\\ 
4 & 1 & 1024 & 20 & $4 \dx 4 \dx 128$ & $1 \dx 1 \dx 1024$ & 8.64MB & 83.9MF & 9.71 & $20 \dx 2048 \dx 1024$\\ 
3 & 1 & 1024 & 1 & $6 \dx 6 \dx 384$ & $6 \dx 6 \dx 1024$ & 14.4MB & 255MF & 17.7 & $36 \dx 3456 \dx 1024$\\ 
3 & 1 & 1024 & 5 & $6 \dx 6 \dx 384$ & $6 \dx 6 \dx 1024$ & 15.2MB & 1.27GF & 84.0 & $180 \dx 3456 \dx 1024$\\ 
3 & 1 & 1024 & 20 & $6 \dx 6 \dx 384$ & $6 \dx 6 \dx 1024$ & 18.2MB & 5.10GF & 280 & $720 \dx 3456 \dx 1024$\\ 
1 & 1 & 4096 & 1 & $1 \dx 1 \dx 4096$ & $1 \dx 1 \dx 4096$ & 67.2MB & 33.6MF & 500m & $1 \dx 4096 \dx 4096$\\ 
1 & 1 & 4096 & 5 & $1 \dx 1 \dx 4096$ & $1 \dx 1 \dx 4096$ & 67.3MB & 168MF & 2.49 & $5 \dx 4096 \dx 4096$\\ 
1 & 1 & 4096 & 20 & $1 \dx 1 \dx 4096$ & $1 \dx 1 \dx 4096$ & 67.8MB & 671MF & 9.90 & $20 \dx 4096 \dx 4096$\\ 
6 & 1 & 4096 & 1 & $6 \dx 6 \dx 256$ & $1 \dx 1 \dx 4096$ & 151MB & 75.5MF & 500m & $1 \dx 9216 \dx 4096$\\ 
6 & 1 & 4096 & 5 & $6 \dx 6 \dx 256$ & $1 \dx 1 \dx 4096$ & 151MB & 377MF & 2.50 & $5 \dx 9216 \dx 4096$\\ 
6 & 1 & 4096 & 20 & $6 \dx 6 \dx 256$ & $1 \dx 1 \dx 4096$ & 152MB & 1.51GF & 9.93 & $20 \dx 9216 \dx 4096$\\ 


==> op-info-tab.tex <==
1 & 1 & 256 & 20 & $13 \dx 13 \dx 256$ & $13 \dx 13 \dx 256$ & 7.19MB & 443MF & 61.7 & $3380 \dx 256 \dx 256$\\ 
3 & 1 & 256 & 20 & $13 \dx 13 \dx 128$ & $13 \dx 13 \dx 256$ & 7.55MB & 3.99GF & 528 & $3380 \dx 2304 \dx 256$\\ 
7 & 2 & 96 & 20 & $205 \dx 205 \dx 3$ & $100 \dx 100 \dx 96$ & 86.9MB & 5.64GF & 64.9 & $200000 \dx 147 \dx 96$\\ 


==> sgemm-SD820-eff-tab.tex <==
$128 \dx 128 \dx 128$ & \verb|sgemm_simd| & 264us & 15.9GF/s & 7.22\\ 
$256 \dx 256 \dx 256$ & \verb|sgemm_simd| & 507us & 66.2GF/s & 30.1\\ 
$384 \dx 384 \dx 384$ & \verb|sgemm_simd| & 2.09ms & 54.3GF/s & 24.7\\ 
$512 \dx 512 \dx 512$ & \verb|sgemm_simd| & 3.61ms & 74.3GF/s & 33.8\\ 
$768 \dx 768 \dx 768$ & \verb|sgemm_simd| & 11.6ms & 78.0GF/s & 35.5\\ 
$1024 \dx 1024 \dx 1024$ & \verb|sgemm_simd| & 26.8ms & 80.1GF/s & 36.4\\ 
$1536 \dx 1536 \dx 1536$ & \verb|sgemm_simd| & 89.1ms & 81.4GF/s & 37.0\\ 
$2048 \dx 2048 \dx 2048$ & \verb|sgemm_simd| & 223ms & 77.1GF/s & 35.0\\ 


==> sgemm-cublas-eff-tab.tex <==
$128 \dx 128 \dx 128$ & \verb|cublas_sgemm| & 64.2us & 65.3GF/s & 990m\\ 
$256 \dx 256 \dx 256$ & \verb|cublas_sgemm| & 62.5us & 537GF/s & 8.14\\ 
$384 \dx 384 \dx 384$ & \verb|cublas_sgemm| & 76.5us & 1.48TF/s & 22.4\\ 
$512 \dx 512 \dx 512$ & \verb|cublas_sgemm| & 121us & 2.22TF/s & 33.7\\ 
$768 \dx 768 \dx 768$ & \verb|cublas_sgemm| & 218us & 4.16TF/s & 63.1\\ 
$1024 \dx 1024 \dx 1024$ & \verb|cublas_sgemm| & 625us & 3.44TF/s & 52.1\\ 
$1536 \dx 1536 \dx 1536$ & \verb|cublas_sgemm| & 1.37ms & 5.29TF/s & 80.1\\ 
$2048 \dx 2048 \dx 2048$ & \verb|cublas_sgemm| & 3.56ms & 4.83TF/s & 73.1\\ 


==> sgemm-eff-tab.tex <==
$64 \dx 64 \dx 64$ & \verb|sgemm| & 149us & 3.52GF/s & 53.3m\\ 
$128 \dx 128 \dx 128$ & \verb|sgemm| & 1.02ms & 4.10GF/s & 62.2m\\ 
$256 \dx 256 \dx 256$ & \verb|sgemm| & 9.39ms & 3.57GF/s & 54.2m\\ 
$384 \dx 384 \dx 384$ & \verb|sgemm| & 30.9ms & 3.66GF/s & 55.5m\\ 
$512 \dx 512 \dx 512$ & \verb|sgemm| & 73.8ms & 3.64GF/s & 55.1m\\ 
$768 \dx 768 \dx 768$ & \verb|sgemm| & 252ms & 3.60GF/s & 54.5m\\ 
$1024 \dx 1024 \dx 1024$ & \verb|sgemm| & 601ms & 3.57GF/s & 54.2m\\ 
$1536 \dx 1536 \dx 1536$ & \verb|sgemm| & 2.10s & 3.45GF/s & 52.2m\\ 


==> sgemm-info-tab.tex <==
197KB & 4.19MF & 21.3 & $128 \dx 128 \dx 128$\\ 
786KB & 33.6MF & 42.7 & $256 \dx 256 \dx 256$\\ 
1.77MB & 113MF & 64.0 & $384 \dx 384 \dx 384$\\ 
3.15MB & 268MF & 85.3 & $512 \dx 512 \dx 512$\\ 
7.08MB & 906MF & 128 & $768 \dx 768 \dx 768$\\ 
12.6MB & 2.15GF & 171 & $1024 \dx 1024 \dx 1024$\\ 
28.3MB & 7.25GF & 256 & $1536 \dx 1536 \dx 1536$\\ 
50.3MB & 17.2GF & 341 & $2048 \dx 2048 \dx 2048$\\ 


==> sgemm-titanX-boda-eff-tab.tex <==
$128 \dx 128 \dx 128$ & \verb|sgemm| & 35.9us & 117GF/s & 1.77\\ 
$256 \dx 256 \dx 256$ & \verb|sgemm| & 59.4us & 565GF/s & 8.56\\ 
$384 \dx 384 \dx 384$ & \verb|sgemm| & 82.0us & 1.38TF/s & 20.9\\ 
$512 \dx 512 \dx 512$ & \verb|sgemm| & 133us & 2.02TF/s & 30.5\\ 
$768 \dx 768 \dx 768$ & \verb|sgemm| & 261us & 3.47TF/s & 52.6\\ 
$1024 \dx 1024 \dx 1024$ & \verb|sgemm| & 622us & 3.45TF/s & 52.3\\ 
$1536 \dx 1536 \dx 1536$ & \verb|sgemm| & 1.70ms & 4.27TF/s & 64.6\\ 
$2048 \dx 2048 \dx 2048$ & \verb|sgemm| & 4.31ms & 3.99TF/s & 60.4\\ 

